Improving Learning-to-Defer Algorithms Through Fine-Tuning

The ubiquity of AI leads to situations where humans and AI work together, creating the need for learning-to-defer algorithms that determine how to partition tasks between AI and humans. We work to improve learning-to-defer algorithms when paired with specific individuals by incorporating two fine-tuning algorithms and testing their efficacy using both synthetic and image datasets. We find that fine-tuning can pick up on simple human skill patterns, but struggles with nuance, and we suggest future work that uses robust semi-supervised to improve learning.

==> 2022_neurips_human_machine_decision_collaboration/lincoln/abstract.tex <==
\begin{abstract}
AI-based systems are used in tandem with humans across a variety of fields including healthcare and criminal justice. 
Maximizing system performance in these situations requires AI to understand the strengths limitations of humans, and allocate tasks accordingly. 
To do this, we build on learning-to-defer models, which allow AI to determine when to defer to humans, to make these models individual specific. 
Doing so allows for finer-grained deference, potentially improving system performance. 
We first outline two strategies for fine tuning, and display the efficacy of individual-specific deference using a synthetic autonomous-vehicle dataset. 
We then conduct experiments using the CIFAR10 image classification task, showing that in some situations, using individual-specific models allows AI to better understand human performance. 
However, we find that this improvement in understanding does not correlate with an improvement in system performance. 
This is potentially due to weak learning algorithms; we propose directions to mitigate this issue and plan for future experiments. 
\end{abstract}

==> 2022_neurips_human_machine_decision_collaboration/lincoln/conclusion.tex <==
\section{Conclusion}
We explore the use of individual-specific human-AI collaboration algorithms. 
We find that the use of individual-specific algorithms can improve expert accuracy rates, and in some cases, improve system performance. 
However, for real experts, improving system performance is difficult due to weaknesses in the learning algorithm. 
We propose future work which rectifies these issues in addition to new experiments. 

==> 2022_neurips_human_machine_decision_collaboration/lincoln/corrupted.tex <==
\section{Corrupted Image recognition}
\subsection{Task Introduction}
What is CIFAR10C? 
\subsection{Data Collection}
How do we collect data for CIFAR10C? 
\subsection{CIFAR10C Data Analysis}
What do machine errors look like on CIFAR10C? What about human errors? We could either have one annotator, or multiple, and fine tune.
\subsection{Experiment Setup}
How do we run the experiment on CIFAR10C. 
\subsection{Results}
What are the results? What does this mean for robustness more generally? 

==> 2022_neurips_human_machine_decision_collaboration/lincoln/discussion.tex <==
\section{Discussion}
\subsection{Limitations}
Our work investigates the use of individual-specific human-AI collaboration algorithms. 
Our results were tested on several annotators and synthetic experts, but could have been expanded, both in terms of the number of trials, and the number of experts. 
Additionally, our semi-supervised learning might not have been robust enough to pick up on expert patterns, and so could be improved through better algorithms. 
In light of this, we discuss future work that builds on our current work. 

\subsection{Future Work}
We explore three avenues for future work. 

\subsubsection{Improved semi-supervised learning algorithms}
As covered in section~\ref{sec: methods}, the problem of incorporating fine tuning to make algorithms individual-specific can be viewed as a form of semi-supervised learning. 
As such, while we have employed self-training algorithms, more sophisticated graph-based algorithms could yield improvements in performance by learning underlying expert patterns. 
Additionally, unlabeled data could be utilized by enforcing an entropy regularization term in the loss function, so to minimize the entropy of unlabeled points while maximizing accuracy on labeled points. 

\subsubsection{Jeopardy Experiments}
To explore the use of human-AI deference algorithms for text datasets, we plan on conducting experiments using the jeopardy question answering dataset~\cite{jeopardy}. 
Individuals vary on skill-set for different types of questions - for example, some people are good at literature, while others are good at science. 
AI models should recognize this, and defer to humans on their strong subjects, while taking over on their weak subjects. 
Doing so potentially requires the use of topic modelling to identify topics, which can be used as inputs to a deep learning model. 
Additionally, surveying expert skill at a topic is a challenge due to incomplete information, as players who might know a topic could fail to buzz in time.
To address this issue, we plan to use some type of imputation to determine confidences on unknown questions. 

\subsubsection{Corrupted Dataset}
Individual-specific fine tuning can be used to explore human robustness on image recognition tasks. 
The CIFAR10C dataset is a corruption of the CIFAR10 dataset, and has been shown to be more difficult for humans~\cite{hendrycks2019robustness}. 
Testing a human-AI collaboration algorithm on this dataset would yield insight into how well human-AI tandems work in the presence of corruptions, and whether humans and AIs are robust to different types of corruptions. 
However, doing so first requires a human-annotated version of the CIFAR10C dataset, which can potentially be collected through MTurk or from volunteers. 
The experiment serves as a way to explore AI predictions when subject to out-of-domain data. 

==> 2022_neurips_human_machine_decision_collaboration/lincoln/driving.tex <==
\section{Motivating Experiments - Autonomous Vehicles}
\label{sec:driving}
Human-AI collaboration naturally arises in the realm of autonomous vehicles, and while the quality of these vehicles has improved recently, they still lag behind humans.
We allow autonomous vehicles to defer to humans depending on environmental circumstances, and show that fine tuning deference algorithms for individual humans reduces trip durations. 
We first develop a synthetic dataset, then describe our results. 

\subsection{Experimental Setup}
We consider the problem of driving a vehicle under rain and darkness conditions. 
Specifically, we consider vehicle deferral for a given driver, $i$, given raining conditions, $0 \leq r \leq 1$, and darkness conditions, $0 \leq d \leq 1$.
Our dataset consists of $n$ total drivers, each of whom have a mean driving time, $\mu \sim \mathrm{Poisson(35)}$, a rain driving time, $\mu_r \sim \mathrm{Poisson(5)}$, and a darkness driving time, $\mu_d \sim \mathrm{Poisson(5)}$. 
Given $\mu$, $\mu_r$, $\mu_d$, the amount of time necessary to drive a trip in conditions $(r,d)$ is distributed according to 

\begin{equation} 
\mathcal{N}(\mu,\sigma) + r \mathcal{N}(\mu_r,\sigma_r) +  d \mathcal{N}(\mu_d,\sigma_d) 
\end{equation} 

We generate $k$ such trips for each driver; for drivers $j \neq i$, the points are for training, while for driver $i$, the points are split equally between fine tuning and testing. 
During deferral, autonomous vehicles have three options: they can defer to humans, drive independent of conditions in time $\mathcal{N}(\mu_a,\sigma_a)$, or dependent on the conditions in time $\mathcal{N}(\mu_b,\sigma_b) + r \mathcal{N} (\mu_x,\sigma_x) + d \mathcal{N} (\mu_y,\sigma_y)$, where $\mu,\sigma$ are constants. 
This forces autonomous vehicles to learn both a rejector and classifier function, emulating the joint classification-deference problem. 
To assist with learning, an additional $l$  unlabeled $(r,d)$ pairs are presented, and time value predictions are imputed, which follows our method from section ~\ref{sec: methods}. 
For our experiments, we use $\sigma=5$, $\sigma_r=\sigma_d=2$, $\mu_a = 45$, $\sigma_a = .001$, $\mu_b = 40$, $\sigma_b = 5$ $\mu_x = \mu_y = 5$, $\sigma_x = \sigma_y = 2$.


\begin{figure*}
    \centering
    \includegraphics[width=400pt]{images/driving.png}
    \caption{Distribution of time taken with/without fine-tuning, and optimally. Each data point represents the average duration when fine tuning on one driver, over $128$ testing trips. Fine tuning out performs not fine tuning by 30 seconds, showing that fine tuning can assist}
    \label{fig:driving}
\end{figure*}

\subsection{Experimental Results}
We generate $k=256$ trips for $n=10$ drivers, and create an additional $l=1024$ unlabeled rides. 
We train an expert prediction network and a rejector function, and compute time taken for each trip. 
We use a simple feed-forward neural network to model both the rejector-classifier, and the human model. 
To analyze the results, we compute two metrics: ideal time, which chooses as if trip durations are known a priori, thereby ignoring randomness, and known mean, which selects deference based on $\mu$ values. 
Both of these serve as lower bounds on average trip duration. 

We simulate $1000$ different sets of $10$ drivers, and for each, compute the average trip duration, plotting them on figure~\ref{fig:driving}. 
We find that, through fine tuning, we can reduce the average trip duration by 30 seconds, while perfectly learning the mean can reduce trip durations by 2 minutes 30 seconds. 
Therefore, fine tuning reduces trip duration error by $20\%$, and our results are significant with $p<.001$. 
While the median between fine tune and no fine tune are close, the averages are wider apart due to large outliers when not fine tuning. 


==> 2022_neurips_human_machine_decision_collaboration/lincoln/image.tex <==
\section{CIFAR Experiments}
We use the CIFAR image recognition task to asses the impact of fine tuning on human-AI collaboration, using both synthetic and real-world human data. 
We discuss our mixed results and propose next steps. 

\subsection{CIFAR10 dataset}
The CIFAR10 image recognition task asks users to classify 32x32 images into one of ten non-overlapping categories~\cite{krizhevsky2009learning}. 
Human performance on the task in the low to mid 90s, while machine performance has exceeded human performance, and is around $99\%$~\cite{foret2020sharpness}. 
To show the efficacy of human-AI collaboration, we reduce the number of training epochs, so machine performance is at $94\%$. 
We begin by analyzing human performance by utilizing the CIFAR10H dataset, where 50 humans label each test image from CIFAR10~\cite{peterson2019human}. 
We find that, while aggregate human performance is in the mid 90s, human performance varies by class label, ranging from deer at $90\%$ to horse at $98\%$ (figure ~\ref{fig:class}). 
Accuracy differences across classes implies that machine takeover on human-weak classes can improve classification, assuming humans and machines have different accuracy profiles, which is also a consequence of section~\ref{sec:lemma1}. 

\subsection{Manifold exploration}
We investigate CIFAR10 images to determine if differences between easy and hard images are learnable. 
To do this, we apply the PCA dimensionality reduction algorithm to images, and analyze the accuracies of dimensionality reduced points.  
We color points by accuracy, binning accuracies into groups rounded to the nearest tenth, and find that accuracy correlates with the PCA x axis. 
The PCA plot hints at the idea that some fundamental component of an image correlates with accuracy, and so identifying easy and hard images is a feasible task. 

\subsection{Synthetic Experts}
To test the effect of fine tuning in a controlled setting, we develop synthetic experts, and consider their effect on human-AI collaboration. 
These experts are parameterized by the value $k$, which indicates perfect accuracy on the first $k$ image classes, and random guesses on the last $10-k$. 
For example, we would expect a $k=10$ expert to achieve $100\%$ accuracy, and a $k=5$ expert to achieve $50\%+50\%\times10\% == 55\%$ accuracy. 
Each synthetic expert annotates $500$ data points, $250$ of which are for fine tuning, and the rest are for testing. 
We use real human data for training, and use synthetic expert for fine tuning. 

We describe our procedure below; the procedure is also described in section~\ref{sec: methods}. 
We begin by training an expert prediction function that predicts expert success on a problem using a WideResNet model, which outputs $0$ if correct, and $1$ otherwise. 
We train on aggregate human data, then fine tune on half the synthetic expert data. 
After training the expert prediction function, we impute predictions on the 50k training labels, and use the combined data to train a rejector. 
The rejector is an 11 class WideResNet model, which outputs 0-9 to predict a class, and 10 to defer. 
We evaluate the rejector by running it over test data points and comparing system accuracy. 
\subsection{Real Annotator Experiments} 
We run experiments to determine the impact of fine tuning on individual annotators. 
Each annotator for the CIFAR10H dataset annotates 200 images; we aim to optimize for these annotators by fine tuning on 100 images and testing on the other 100. 
Our setup is similar to the synthetic experiments, except swapping synthetic with real experts. 
We repeat this for 11 different annotators and asses the impact on system accuracy. 
\subsection{Experimental Setup}
We run both real and synthetic expert experiments, trying $k=0 \cdots 10$ for synthetic experiments, and using 11 different annotators for real annotators. 
We measure deference rate and accuracy on deferences. 
We try three different types of fine tuning: no fine tuning, baseline fine tuning, and self training. 
\subsection{Results}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=200pt]{images/human_model_accuracy_synthetic.png}
    \includegraphics[width=200pt]{images/human_model_accuracy_annotator.png}
    \caption{We plot human model accuracies for synthetic and real annotator collaborations. We find that introducing fine tuning assists human model accuracies for synthetic data but not real annotators. }
    \label{fig:human_accuracy}
\end{figure}
We overview our biggest takeaways from the synthetic and real annotator experiments
\begin{enumerate}
    \item \textbf{Introduction of fine tuning can improve expert prediction} - We see that, in the case of synthetic experts, the introduction of fine tuning improves expert prediction accuracy, particularly for low values of K (figure~\ref{fig:human_accuracy}). 
    However, such a pattern fails to hold when dealing with real annotators, as fine tuning fails to outperform not fine tuning. 
    We believe these results occur due to the situation learnability; synthetic experts pose an easier challenge when compared to real annotators, who have more nuanced strengths and weaknesses. 
    Such results could also be due to dataset sizes, as annotators only have 100 fine tuning points, when compared with 256 for synthetic experts. 
    \item \textbf{Improvements in expert prediction accuracy fail to improve system accuracy} - We see that for both synthetic and real annotator data that improvements in expert prediction accuracy fail to result in system accuracy improvements. 
    This is partially explained by low deference rates leading to reliance on system rather than human classification. 
    However, there still are situations where high deference and expert accuracy rates are not aligned with high system accuracy ,and the reasons why are still unknown. 
    \item \textbf{Deference accuracies are high across the board} - For both no fine tuning and the two types of fine tuning, human accuracy on deferred examples is consistently higher than deferring randomly, showing that expert models successfully learn something about human performance.
    Of note is high deference accuracies for low values of $k$ on synthetic experts with no fine tuning. 
    This result is counter-intuitive, as the lack of fine tuning on experts so different from aggregate humans should imply poor performance. 
    The reason this occurs is unknown and could potentially be due to a bug in the code. 
\begin{figure}[!ht]
    \centering
    \includegraphics[width=200pt]{images/system_accuracy_synthetic.png}
    \includegraphics[width=200pt]{images/system_accuracy_annotator.png}
    \caption{We plot system accuracy for synthetic and real annotator setups. Despite improvements in human accuracy, we find that system accuracy fails to consistently increase when using fine tuning, for both synthetic and real annotators. }
    \label{fig:system_accuracy}
\end{figure}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=200pt]{images/deference_accuracy_synthetic.png}
    \includegraphics[width=200pt]{images/deference_accuracy_annotator.png}
    \caption{We compute accuracy on deferred examples, and find that for synthetic experts, deference accuracy is consistently higher than guessing. However, this is true for both with and without fine tuning, which is strange. }
    \label{fig:human_accuracy}
\end{figure}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=200pt]{images/synthetic_accuracy_improvements.png}
    \caption{We plot how improvements in human accuracy impact system accuracy. We find a generally positive pattern, as improvements in human accuracy lead to improvements in system accuracy, though the effect is not very large, and there is a fair amount of noise. Therefore, improvements in human accuracy might contribute to small improvements in system accuracy, but these trends are incredibly noisy.  }
    \label{fig:human_accuracy}
\end{figure}

\end{enumerate}

\subsection{Discussion} 
Our CIFAR experiment results are largely mixed and demonstrate that the rejector understands human performance, but not sufficiently well to improve system performance. 
We believe the problem is due to the learning algorithm rather than the nature of the problem, as sufficiently good learning algorithms should be able to pickup on differences in accuracy profiles. 
Potential steps to mitigate this issue include the use of graph-based semi supervised learning algorithms, and the expansion of fine tuning datasets. 
We additionally find a tradeoff between the amount of data available, and specificity of data for the model. 
In particular, we have a small amount of individual-specific data, which is a better fit, and a large amount of aggregate human data, which is a worse fit, which leads to fine tuning only assisting in certain scenarios. 


==> 2022_neurips_human_machine_decision_collaboration/lincoln/introduction.tex <==
\section{Introduction}
The rise of neural technologies has led to the adoption of AI-based solutions for human-facing tasks in fields such as health care and criminal justice. 
Examples of this include the COMPAS recidivism algorithm, which uses AI to predict recidivism probabilities for defendants~\cite{washington2018argue}. 
Many times, these algorithms work alongside humans, and are tasked with determining whether to answer a problem or to defer. 
\\
Determining when to defer, also known as learning to defer, is a challenging problem explored by prior work. 
Determining this relies not only on model confidences, but its interpretation of human expertise. 
Numerous studies~\cite{mozannar2020consistent,raghu2019algorithmic,wilder2020learning} have developed methods to learn when to defer based off human and machine uncertainty.
This includes both confidence-based methods~\cite{raghu2019algorithmic} and joint learning methods~\cite{mozannar2020consistent,okati2021differentiable}, which learn rejector and classifier functions simultaneously. 
Other work in this space includes multi-agent deferral~\cite{keswani2021towards} and human initiated deferral~\cite{bansal2021most}. 
\\
While much of the attention has been focused on optimal learning methods, less attention has been focused on understanding human skill. 
Human skill varies between individuals, and so understanding humans skill in aggregate might not be applicable to instances where individual skill differs from aggregate skill. 
Allowing for deference algorithms to be individual-specific can mitigate this problem, allowing for a more nuanced view of human skill, and potentially improving system performance. 
To tackle this problem, we develop two fine tuning methods which allow for human-AI models to be individual-specific.
We prove theoretical bounds on the error when using joint human-AI systems. 
%that, with sufficient knowledge of human and AI skills, human-AI joint models  out-perform humans or AI models independently, motivating the need to understand human skill. 
As a simple example, we develop a synthetic dataset based on autonomous driving, and show that fine tuning for individuals reduces average trip duration. 
We then run experiments comparing performance using different types of fine tuning for the CIFAR10 image recognition task,using both real and synthetic humans~\cite{krizhevsky2009learning}. 
\\
Our contributions are as follows. 
We (1) develop two fine tuning methods which allow for human-AI models to be individual specific, (2) show the application of this model to autonomous driving and image recognition tasks, and (3) prove bounds on the relationship between human-AI calibration error and system error.
\begin{figure*}
    \centering
    \includegraphics[width=400pt]{images/datapoints_5.png}
    
    \caption{We describe the problem, by noting what type of data is available. Our two fine tuning methods use these data points to learn a rejector and classifier function}
    \label{fig:datapoints}
\end{figure*}

==> 2022_neurips_human_machine_decision_collaboration/lincoln/main.tex <==
\input{meta}
\pdfinfo{
/Title (Human-Machine Joint Collaboration)
/Author (Naveen Raman, Michael Yee)
/TemplateVersion (2021.2)
} 


\setcounter{secnumdepth}{2} 
\title{(DRAFT) Human-Machine Joint Collaboration}
\author{
    Naveen Raman \textsuperscript{\rm 1, \rm 2}, Michael Yee \textsuperscript{\rm 1} 
    \\
}
\affiliations{
    \textsuperscript{\rm 1} MIT Lincoln Labs 
    \textsuperscript{\rm 2} University of Maryland, College Park \\
}


\begin{document}

\maketitle

\makeatletter{\renewcommand*{\@makefnmark}{}
\footnotetext{\\ DISTRIBUTION STATEMENT A. Approved for public release. Distribution is unlimited. \\ \\ This material is based upon work supported by the Under Secretary of Defense for Research and Engineering under Air Force Contract No. FA8702-15-D-0001. Any opinions, findings, conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the Under Secretary of Defense for Research and Engineering.}\makeatother}

\input{sections/abstract}
\input{sections/introduction}
\input{sections/related}
\input{sections/problem}
\input{sections/methods}
\input{sections/theory}
\input{sections/driving}
\input{sections/image}
\input{sections/discussion}
\input{sections/conclusion}

\clearpage
\bibliographystyle{aaai}
\bibliography{references.bib}

\end{document}



==> 2022_neurips_human_machine_decision_collaboration/lincoln/methods.tex <==
\section{Learning algorithms}
We describe a learning algorithm to learn rejectors and classifiers jointly, then describe our two fine tuning methods. 
\label{sec: methods}
\subsection{State of the art human-AI collaboration}
We describe the state of the art human-AI collaboration algorithm, taken from prior work~\cite{mozannar2020consistent}. 
The algorithm does not fine tune on human specific data, and so $n=0$. 
Instead it trains and tests on different splits of the aggregate human data. 
The algorithm proceeds as follows: we first train an artificial  human, $\hat{h}$ from human performance on some subset of the human labeled data, $c_1 \cdots c_b$ with human predictions $e_1 \cdots e_b$, using $c_{b+1} \cdots c_{l}$ for testing. 
Given an input, $c_i$, the function $\hat{h{(c_i)}}$ learns whether a human will answer $c_i$ correctly, returning 0 if the do, and 1 if they don't. 
After learning on $c_1 \cdots c_b$, imputed labels are generated for the whole training set by running $\hat{h}$ over $t_{1} \cdots t_n$. 
Imputation allows for predicted human labels on all test points, which is used when training $m$, the classifier, and $a$, the rejector. 
To improve system performance, $a$ and $m$ are learned simultaneously, so if the classification problem is for $k$-classes, then we learn a $k+1$ classification function, where the ${k+1}^{\textrm{st}}$ class indicates deference to humans. 
For each data point, predictions are made using the augmented machine function (k+1 classes) $\bar{m}$, and then optimized over a modified cross-entropy loss function~\cite{mozannar2020consistent}.
The loss function asses a penalty of $\alpha$ for deferring to humans, and a penalty of $1$ for incorrect predictions. 
After training using this loss function, the augmented machine function, $\bar{m}$, is run over the test dataset, $c_{b+1} \cdots c_{l}$, and evaluated based on system accuracy and loss. 
Full details of this algorithm is found in past work~\cite{mozannar2020consistent}. 
\subsection{Semi-supervised learning}
Our problem can be viewed as an extension of semi supervised learning, which aims to learn a classifier given both labeled and unlabeled data. 
In our scenario, we're given both unlabeled image data, image data labeled by other humans, and image data labeled by a specific individual.
Therefore, the challenge is to incorporate both unlabeled and similarly labeled data in an effective manner. 

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=300pt]{images/accuracy_by_class.png}
    \caption{Human accuracy varies by the class, ranging from deer at $90\%$ to horses at $98\%$. Machine assistance on deer classes can greatly improve performance. }
    \label{fig:class}
\end{figure*}

\subsection{Baseline Fine tuning} 
We incorporate elements of fine tuning into the baseline methodology to improve system accuracy for specific humans. 
We primarily modify the training loop by adding an extra an extra loop to train on the fine tuning set, $x_1 \cdots x_{n/2}$. 
To account for class imbalances, which could skew training due to small fine tuning dataset size, we introduce a class-weighting scheme, which weights the loss function by the inverse frequency of each class. 
\subsection{Self Training} 
\begin{figure*}
    \centering
    \includegraphics[width=300pt]{images/cifar_pca.png}
    \caption{We dimensionality reduce CIFAR10 images using the PCA algorithm, and color by human accuracy. Notice that harder images are to the left, and that the difficulty of the image corresponds to the x axis. }
    \label{fig:pca}
\end{figure*}


We adopt the self training algorithm from semi supervised learning as an alternative to the baseline~\cite{chapelle2009semi}. 
For self training, we first train a classifier using $x_1 \cdots x_{n/2}$. 
Using this basic classifier, we predict labels for the unlabeled data points, $t_{1} \cdots t_{a}$, then select the high confidence predictions. 
We use these high confidence points to retrain the classifier, generating a better classifier in the process. 
The advantage of self training is that it uses unlabeled data points to develop a better classifier, leveraging all the available data. 
We employ both baseline fine tuning and self training as fine tuning mechanisms for our image experiments. 
We present a pictorial representation of both algorithms in figure~\ref{fig:fine_tuning}. 

==> 2022_neurips_human_machine_decision_collaboration/lincoln/problem.tex <==
\section{Problem Statement}
We define the problem of human-AI collaboration for classification. 
That is, given a classification task, $T$, which consists of data points $x_{1} \cdots x_{n}$, and human and AI agents, we consider the problem of apportioning $x_{1} \cdots x_{n}$ to maximize system performance. 
Each point is solved by a human, $h(x_i)$, or a machine, $m(x_i)$. 
Our aim to maximize overall system accuracy, so if we let $a(x_i)=0$ if a human answers, and $a(x_i)=1$ otherwise.  

Rather than viewing human data as arising from a distribution of skill, we view human data as arising from a distribution of distributions. 
That is, each individual has their own distribution of skills, and the parameters for that distribution are itself taken from a distribution. 
We make these distributions explicit in section~\ref{sec:driving}, and provide a visual of these data points in figure~\ref{fig:datapoints}. 

Following previous work, we aim to learn both the deference function $a$ and the classifier $m$ simultaneously~\cite{mozannar2020consistent}. 
To learn $a$ and $m$, we consider two types of training points: human-annotated training points and truth-labeled training points.
Truth-labeled points are common, and serve as training points for a classifier, while human-annotated training points serve to assess human skill at a task. 
We have training points, $t_{1} \cdots t_{a}$, with truth labels $s_{1} \cdots s_{a}$, but lack human labels. 
We have humans labeled points $c_{1} \cdots c_{l}$ with truth labels $d_{1} \cdots d_{l}$ and human labels $e_{1} \cdots e_{l}$. 
We additionally have points from one individual, who annotated points $x_1 \cdots x_n$ with truth labels $y_1 \cdots y_n$ and human labels $z_1 \cdots z_n$. 
We consider the first $\frac{n}{2}$ individual-specific points to be for fine tuning, and the last $\frac{n}{2}$ to be for testing. 
Therefore, we aim to learn $m$ and $a$ to maximize 
\begin{equation} 
\sum_{i=\frac{n}{2}}^{n}  
\begin{cases} 
      h(x_i)=y_i & a(x_i) = 0 \\
      m(x_i)=y_i & a(x_i) = 1  
   \end{cases}
\end{equation}
We describe the state of the art solution, which lacks fine tuning, then describe our two solutions which use fine tuning. 
\begin{figure*}
    \centering
   \includegraphics[width=250pt]{images/datapoints_6.png}
  \includegraphics[width=250pt]{images/datapoints_7.png}
    \caption{Our two fine tuning methods. The first uses individual-specific data on top of the human model, while the second uses self training to fine tune the model. }
    \label{fig:fine_tuning}
\end{figure*}


==> 2022_neurips_human_machine_decision_collaboration/lincoln/related.tex <==
\section{Related Works}
\textbf{Human-AI Collaboration} - Collaboration between humans and machines has been explored in various domains including finance~\cite{nagar2011making} and healthcare~\cite{patel2019human}. 
Collaboration is beneficial as information from both sources can be combined to make decisions~\cite{nagar2011making}. 
However, collaboration has risks, as algorithmic predictions can anchor and bias human predictions~\cite{vaccaro2019effects}. 
This problem is further exacerbated when AI solutions are accompanied with explanations~\cite{bansal2021does}, as humans are more liable to accept explanations regardless of its veracity. 
However, the problem can be mitigated through the development of human mental models, which acknowledge deficits in AI performance~\cite{bansal2019beyond}. 
The lack of algorithmic transparency makes it difficult for humans to ascertain liability to AI models, complicating the legality of algorithmic decision making~\cite{williams2019rethinking}. \\ \\
\textbf{Learning to defer} - One area of research within human-AI collaboration is learning to defer algorithms, where AI systems defer to humans when unsure. 
For classification problem, the AI system consists of a rejector, which determines deference, and classification, which solves the task. 
One deference strategy is to calculate confidence scores for AI and humans, and defer based on whichever is higher~\cite{raghu2019algorithmic,madras2017predict}. 
However, these approaches ignore the interconnectedness of the rejector and classifier, as AI systems should focus on tasks that are hard for humans, and to solve this, prior work has developed a joint learning algorithm to simultaneously learn a rejector and classifier through the use of a new loss function~\cite{wilder2020learning,mozannar2020consistent}. 
Prior work has shown that learning to defer algorithms are proven to outperform humans and machines separately in the case of SVMs~\cite{de2021classification}. 
Extensions to the learning to defer algorithm include algorithms for multiple experts~\cite{keswani2021towards} and for human-initiated deferral~\cite{bansal2021most}. 
Our work most directly builds on work by~\citet{mozannar2020consistent}, and answers an open problem from~\citet{de2021classification} to develop human-AI collaboration algorithms for specific humans via fine-tuning


==> 2022_neurips_human_machine_decision_collaboration/lincoln/text.tex <==
\section{Jeopardy Question Answering}
We extend our human-machine collaboration to a text-based question-answering task. 

\subsection{Dataset}
We use the Jeopardy! dataset to determine human and machine performance on question answering. 
We train a BERT-based model to predict human accuracy (and response time?) based on responses to jeopardy questions. 

\subsection{Data analysis}
We look at the data we collected, and the errors made by humans. 

\subsection{Experiment Setup}
We compare joint human-machine models to human and machine-only model on the text dataset, and also see how well we can fine tune. 

\subsection{Experiment Results} 
We find that, for both image and text-based systems, the inclusion of a human in the loop improves system accuracy. 

==> 2022_neurips_human_machine_decision_collaboration/lincoln/theory.tex <==
\section{Impact of human models}
We present and prove two theorems detailing the impact of human models.
We first detail our problem setup, then prove our two theorems. 

\subsection{Problem Setup} 
We consider the problem of characterizing $n$ inputs $x_1, x_2 \cdots x_n$, with labels $y_1, y_2, \cdots x_n$.
For each input, humans output a label $h(x_{i})$, with a confidence $c_{H}(x_i)$.
Similarly, for AI-based machines, they output a label $m(x_{i})$ with confidence $c_{M}(x_{i})$. 
We calibrate confidences, so that the calibrated confidence for humans is $g_{H}(c_{H}(x_i))$ and for machines $g_{M}(c_{M}(x_i))$. 
Humans and machines have true confidences, $p_{H}(x_i)$ and $p_M(x_i)$, so that the probability of a human answering $x_i$ correctly is $p_{H}(x_i)$. 
We define calibration so that the distribution of errors after calibration, $p_{H}(x_i)-g_{H}(c_{H}(x_i))$ has $\mu=0$ and $\sigma=\epsilon$ (and similarly for machines). 
In other words, calibrated confidence are centered at the true confidence, with a standard deviation of $\epsilon$. 

We now define the joint human-machine system. 
This system takes in $x_i$, and decides whether to give the problem to humans or machines, based on $g_{H}(c_{H}(x_i))$ and $g_{M}(c_{M}(x_i))$. 

\subsection{Model error rates}
Our first theorem demonstrates the relationship between model calibration and model error. 
\\ 
\textbf{Lemma:} The probability of misclassification is $\leq \frac{2\epsilon^{2}}{(p_{H}(x_i)-p_{M}(x_i))^{2}}$ \\ 
\textbf{Proof:}
Without loss of generality, assume $p_{H}(x_i) > p_{M}(x_i)$. 
The probability of an incorrect classification is $\mathrm{Pr}(g_{H}(c_{H}(x_i))<g_{M}(c_{M}(x_i)))$
Assuming independence between the distributions, we let $X = g_{M}(c_{M}(x_i)) - g_{H}(c_{H}(x_i)) = (g_{M}(c_{M}(x_i)) - p_{M}(x_i)) - (g_{H}(c_{H}(x_i)) - p_{H}(x_i)) + (p_{M}(x_i) - p_{H}(x_i))$, and determine $\mathrm{Pr}(X>0)$. 
$X$ is centered at $p_M(x_i) - p_{H}(x_i)$, so $\mathrm{Pr}(X>0) \leq \mathrm{Pr}(|X-(p_{M}(x_i)-p_{H}-x_{i})| \geq (p_{H}(x_i) -p_{M}(x_i)))$
By Chebyshev's inequality, we find $\mathrm{Pr}(|X-(p_{M}(x_i)-p_{H}(x_i))| \geq (p_{H}(x_i) -p_{M}(x_i))) \leq \frac{2 \epsilon^{2}}{(p_{H}(x_i)-p_{M}(x_i))^{2}}$, as $\mathrm{Var}(X) = 2 \epsilon^{2}$
\\
\\
\begin{comment} 
\subsection{Improvement over independent humans/machines}
\label{sec:lemma2}
We next compare errors due to misclassification with errors arising from only using human or machine predictions. 
\textbf{Lemma:} If neither humans nor AI Pareto dominate, then human-AI combination outperforms either independently \\ 
\textbf{Proof:}
We suppose that, for each $i$, $p_{H}(x_i)$ and $p_{M}(x_i)$ are randomly sampled from the uniform distribution $[a_{h},b_{h}]$ and $[a_{m},b_{m}]$, denoting the range of confidences for humans and machines respectively. 
We suppose that $a_{h} \leq a_{m} \leq b_{h} \leq b_{m}$. 
Note that if the uniform distributions do not intersect, that is, $p_{H}(x_i) > p_{M}(x_i)$ for all $i$, then independent human systems outperform joint systems. 
We wish to find the expected loss due to using only human predictions, which is $\mathrm{Pr}(p_{H}(x_i)<p_{M}(x_i))*E[p_{M}(x_i)-p_{H}(x_i)|p_{H}(x_i)<p_{M}(x_i)]$.
Note that the PDF for each uniform distribution is $\frac{1}{b_{h}-a_{h}}$ and $\frac{1}{b_{m}-a_{m}}$
We find this by evaluating a double integral
\begin{equation}
    \begin{aligned}
        \frac{1}{(b_{h}-a_{h})(b_{m}-a_{m})} \int_{a_{h}}^{b_{m}} \int_{a_{h}}^{x} x-y dy dx \\ 
        =  \frac{(b_{m}-a_{h})(\frac{a_{h}^2}{2} - a{h})+\frac{b_{m}}{6}}{(b_{h}-a_{h})(b_{m}-a_{m})}
    \end{aligned}
\end{equation}

The expected error due to misclassification is $E[\epsilon^{2}/(p_{H}(x_{i}) - p_{M}(x_i)) * (p_{H}(x_{i}) - p_{M}(x_i)] = E[\frac{\epsilon^2}{p_{H}(x_{i})-p_{M}(x_i)}] = \frac{\epsilon^{2}}
{E[p_{H}(x_{i})-p_{M}(x_i)]}$. 
We evaluate the denominator to get 
\begin{equation}
    \begin{aligned}
    \int_{a_{m}}^{b_{m}} \int_{a_{h}}^{x} x-y dy dx + \int_{a_{m}}^{b_{m}} \int_{x}^{b_{h}} y-x dy dx = \\ 
    \frac{6 \epsilon^2 (c-d)}{3d^2-3(b+a)(d) + 3c^2-3(b+a)c+2b^2+2ab+2a^2}
    \end{aligned}
\end{equation}

In essence, this means that if we can reduce $\epsilon$ so that it's sufficiently small, and if humans are not dominant on every questions, then combining humans and machines can outperform either independently. 
\end{comment}

==> 2022_neurips_human_machine_decision_collaboration/meta.tex <==
\usepackage{neurips_2021}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors


==> 2022_neurips_human_machine_decision_collaboration/sections/abstract.tex <==
The ubiquity of AI leads to situations where humans and AI work together, creating the need for learning-to-defer algorithms that determine how to partition tasks between AI and humans. 
We work to improve learning-to-defer algorithms when paired with specific individuals by incorporating two fine-tuning algorithms and testing their efficacy using both synthetic and image datasets. 
We find that fine-tuning can pick up on simple human skill patterns, but struggles with nuance, and we suggest future work that uses robust semi-supervised to improve learning.  

==> 2022_neurips_human_machine_decision_collaboration/sections/autonomous.tex <==
\section{Autonomous Vehicle Experiment}
\label{sec:driving}
Human-AI collaboration naturally arises in the realm of autonomous vehicles, which requires deferral to humans depending on environmental circumstances. 
We develop a synthetic dataset based on autonomous driving, and show that fine-tuning learning-to-defer algorithms reduces trip durations. 

\subsection{Experimental Setup}
We consider vehicle deferral for a given driver, $i$, given rain condition, $0 \leq r \leq 1$, and darkness condition, $0 \leq d \leq 1$.
Our dataset consists of $n$ total drivers, each of whom have a mean driving time, $\mu \sim \mathrm{Poisson(35)}$, a rain driving time, $\mu_r \sim \mathrm{Poisson(5)}$, and a darkness driving time, $\mu_d \sim \mathrm{Poisson(5)}$. 
Given $\mu$, $\mu_r$, and $\mu_d$, the amount of time necessary to drive a trip in conditions $(r,d)$ is distributed according to
\begin{equation} 
\mathcal{N}(\mu,\sigma) + r \mathcal{N}(\mu_r,\sigma_r) +  d \mathcal{N}(\mu_d,\sigma_d) 
\end{equation} 

We generate $k$ such trips for each driver; for drivers, $j \neq i$, the points are for training, while for driver $i$, the points are split equally between fine-tuning and testing. 
Autonomous vehicles have three options: they can defer to humans, drive independent of conditions in time $\mathcal{N}(\mu_a,\sigma_a)$, or drive  dependent on conditions in time $\mathcal{N}(\mu_b,\sigma_b) + r \mathcal{N} (\mu_x,\sigma_x) + d \mathcal{N} (\mu_y,\sigma_y)$, where $\mu,\sigma$ are constants chosen to make it possible for the system to reduce average trip time by making accurate defer decisions.
This forces autonomous vehicles to learn both a rejector and classifier function, emulating the joint classification-rejection problem. 
To assist with learning, an additional $l$ unlabeled $(r,d)$ pairs are presented. 
We provide further experimental details in Appendix~\ref{sec:autonomous-appendix}.

\begin{figure*}
    \centering
    \includegraphics[width=250pt]{images/driving.png}
    \caption{Distribution of time taken with/without fine-tuning and ideally. Each data point represents the average trip duration when fine-tuning on one driver, over $128$ testing trips. Fine-tuning outperforms no fine-tuning by 30 seconds, showing that fine-tuning can assist autonomous vehicles.}
    \label{fig:driving}
\end{figure*}


\subsection{Experimental Results}
To analyze the results, we compute the ideal time, which chooses knowing trip durations beforehand and ignores randomness, and known mean, which chooses based on known $\mu$ values.
Both of these serve as lower bounds on average trip duration.

We find that fine-tuning reduces average trip duration by 30 seconds compared to not fine-tuning, while knowing $\mu$ values can reduce trip durations by 2 minutes 30 seconds. 
Fine-tuning reduces trip duration error by $20\%$ (i.e., it achieves $20\%$ of achievable reduction if $\mu$ values were known), and our results are significant with $p<.001$. 
While the medians between the two learning-to-defer methods are close, the means are wider apart due to large outliers when not fine-tuning.

==> 2022_neurips_human_machine_decision_collaboration/sections/cifar.tex <==
\section{CIFAR-10 Experiments}
We use the CIFAR-10 image classification task to assess the impact of fine-tuning on human-AI collaboration, using both synthetic human models and real human annotation data. 

% \subsection{CIFAR10 dataset}
% To show the efficacy of human-AI collaboration, we reduce the number of training epochs, so machine performance is at $94\%$.
% We develop synthetic experts, which classify images based on a parameter $k$, and real experts, which are taken from the CIFAR10H dataset~\cite{peterson2019human}. 
% We begin by analyzing human performance by utilizing the CIFAR10H dataset, where 50 humans label each test image from CIFAR10~\cite{peterson2019human}. 
% We find that, while aggregate human performance is in the mid-90s, human performance varies by class label, ranging from deer at $90\%$ to the horse at $98\%$ (figure ~\ref{fig: class}). 
% Accuracy differences across classes imply that machine takeover on human-weak classes can improve classification, assuming humans and machines have different accuracy profiles, which is also a consequence of section~\ref{sec:lemma1}. 

% \subsection{Manifold exploration}
% We investigate CIFAR10 images to determine if differences between easy and hard images are learnable. 
% To do this, we apply the PCA dimensionality reduction algorithm to images, and analyze the accuracies of dimensionality reduced points.  
% We color points by accuracy, binning accuracies into groups rounded to the nearest tenth, and find that accuracy correlates with the PCA x-axis. 
% The PCA plot hints at the idea that some fundamental component of an image correlates with accuracy, and so identifying easy and hard images is a feasible task. 

\subsection{Experiment Setup}
This task asks users to classify 32x32 images into one of ten non-overlapping categories~\cite{krizhevsky2009learning}. 
We consider the effect of fine-tuning when having synthetic or real experts work with AI image classifiers. 

As in~\cite{mozannar2020consistent}, we create synthetic experts parameterized by $k$, which indicates perfect accuracy on the first $k$ image classes, and random guesses on the last $10-k$. 
Each synthetic expert annotates $500$ images, while real experts annotate $200$ images, which are split $50\%-50\%$ for fine-tuning and testing.
For human expert data, we select 11 annotators from CIFAR-10H~\cite{peterson2019human}.

We begin by training a human performance function $\hat{h}$ to predict expert success on an image, outputting $0$ if correct, and $1$ otherwise.
We train a WideResNet model~\cite{zagoruyko2016wide} on aggregate human data from CIFAR-10H, then fine-tune on data from a single synthetic or real expert.
For self-training, after training $\hat{h}$, we impute predictions on the 50k training labels that lack human predictions, then retrain using high confidence points.
We use the fine-tuned human performance model to learn a combined rejector-classifier, which is an 11-class WideResNet model that outputs 0-9 to predict a class, and 10 to defer.
We evaluate system accuracy over the test images and compare three different approaches: no fine-tuning, baseline fine-tuning, and fine-tuning with self-training.
\subsection{Results}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=150pt]{images/human_model_accuracy_synthetic.png}
    \includegraphics[width=150pt]{images/system_accuracy_synthetic.png}
    \caption{Human model and system accuracy for synthetic annotators. Fine-tuning improves human model accuracy, especially for low values of $k$, though fails to consistently improve system accuracy.}
    \label{fig:human_accuracy}
\end{figure}
Our takeaways from the synthetic and real annotator experiments are:
\begin{enumerate}
    \item \textbf{Fine-tuning can improve expert prediction in some situations}. For synthetic experts, fine-tuning improves human model accuracy, particularly for low values of $k$ (Figure~\ref{fig:human_accuracy}). 
    However, fine-tuning fails to consistently outperform not fine-tuning for real annotators, potentially due to lack of learnability.
    Synthetic experts may pose an easier challenge when compared to real annotators with more nuanced strengths and weaknesses.
    \item \textbf{Correlation between human and system accuracy}. For real experts, when baseline fine-tuning improves human model accuracy, system accuracy also improves $75\%$ of the time.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=150pt]{images/human_model_accuracy_annotator.png}
    \includegraphics[width=150pt]{images/system_accuracy_annotator.png}
    \caption{Human model and system accuracy for real annotators. Fine-tuning doesn't consistently improve human model; however, when it helps, system accuracy also tends to improve.}
    \label{fig:system_accuracy}
\end{figure}
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=200pt]{images/deference_accuracy_synthetic.png}
%     \includegraphics[width=200pt]{images/deference_accuracy_annotator.png}
%     \caption{We compute accuracy on deferred examples, and find that for synthetic experts, deference accuracy is consistently higher than guessing. However, this is true for both with and without fine tuning, which is strange. }
%     \label{fig:human_accuracy}
% \end{figure}
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=200pt]{images/synthetic_accuracy_improvements.png}
%     \caption{We plot how improvements in human accuracy impact system accuracy. We find a generally positive pattern, as improvements in human accuracy lead to improvements in system accuracy, though the effect is not very large, and there is a fair amount of noise. Therefore, improvements in human accuracy might contribute to small improvements in system accuracy, but these trends are incredibly noisy.  }
%     \label{fig:human_accuracy}
% \end{figure}
\end{enumerate}
Our results indicate that fine-tuning can pick up on simple patterns of skill, but struggles with nuance.
We can potentially improve fine-tuning by exploring more sophisticated semi-supervised learning algorithms, such as graph-based techniques~\cite{subramanya2014graph}, which can then boost system accuracy.


==> 2022_neurips_human_machine_decision_collaboration/sections/conclusion.tex <==
\section{Conclusion}
We explore the use of individual-specific human-AI collaboration algorithms. 
We find that tailoring learning-to-defer algorithms to individuals through fine-tuning can improve human model and system accuracy in some situations. However, initial fine-tuning approaches struggle to consistently improve human model performance for real experts, though can improve system performance when they do. We propose investigating more advanced semi-supervised techniques to address this.

==> 2022_neurips_human_machine_decision_collaboration/sections/discussion.tex <==
\section{Discussion}
\subsection{Limitations}
Our work investigates the use of individual-specific human-AI collaboration algorithms. 
Our results were tested on several annotators and synthetic experts, but could have been expanded, both in terms of the number of trials, and the number of experts. 
Additionally, our semi-supervised learning might not have been robust enough to pick up on expert patterns, and so could be improved through better algorithms. 
In light of this, we discuss future work that builds on our current work. 

\subsection{Future Work}
We explore three avenues for future work. 

\subsubsection{Improved semi-supervised learning algorithms}
As covered in section~\ref{sec: methods}, the problem of incorporating fine tuning to make algorithms individual-specific can be viewed as a form of semi-supervised learning. 
As such, while we have employed self-training algorithms, more sophisticated graph-based algorithms could yield improvements in performance by learning underlying expert patterns. 
Additionally, unlabeled data could be utilized by enforcing an entropy regularization term in the loss function, so to minimize the entropy of unlabeled points while maximizing accuracy on labeled points. 

\subsubsection{Jeopardy Experiments}
To explore the use of human-AI deference algorithms for text datasets, we plan on conducting experiments using the jeopardy question answering dataset~\cite{jeopardy}. 
Individuals vary on skill-set for different types of questions - for example, some people are good at literature, while others are good at science. 
AI models should recognize this, and defer to humans on their strong subjects, while taking over on their weak subjects. 
Doing so potentially requires the use of topic modelling to identify topics, which can be used as inputs to a deep learning model. 
Additionally, surveying expert skill at a topic is a challenge due to incomplete information, as players who might know a topic could fail to buzz in time.
To address this issue, we plan to use some type of imputation to determine confidences on unknown questions. 

\subsubsection{Corrupted Dataset}
Individual-specific fine tuning can be used to explore human robustness on image recognition tasks. 
The CIFAR10C dataset is a corruption of the CIFAR10 dataset, and has been shown to be more difficult for humans~\cite{hendrycks2019robustness}. 
Testing a human-AI collaboration algorithm on this dataset would yield insight into how well human-AI tandems work in the presence of corruptions, and whether humans and AIs are robust to different types of corruptions. 
However, doing so first requires a human-annotated version of the CIFAR10C dataset, which can potentially be collected through MTurk or from volunteers. 
The experiment serves as a way to explore AI predictions when subject to out-of-domain data. 

==> 2022_neurips_human_machine_decision_collaboration/sections/introduction.tex <==
\section{Introduction}
The rise of neural technologies has led to the adoption of AI-based solutions for human-facing tasks in fields such as health care~\cite{tran2019patients} and criminal justice~\cite{washington2018argue}.
In some situations, humans and AI collaborate to solve a problem by partitioning tasks so AI solves problems that are difficult for humans. 
Determining task partitions is done through a learning-to-defer algorithm, which uses a human performance model to take human skill into account. 
Numerous studies~\cite{mozannar2020consistent,raghu2019algorithmic,wilder2020learning} have developed learning-to-defer algorithms using confidence-based~\cite{raghu2019algorithmic} and joint learning methods~\cite{mozannar2020consistent,okati2021differentiable}, which learn rejector and classifier functions simultaneously. 

Learning-to-defer algorithms can be used with specific individuals, such as an individual doctor working with an AI to classify X-ray images. 
In these situations, learning-to-defer algorithms can be improved by fine-tuning their underlying human performance models. 
Fine-tuning exploits human skill variation to improve system performance. 
For example, when AI classifies X-ray images, learning-to-defer algorithms should tune to the doctor's expertise. 
We incorporate fine-tuning into learning-to-defer algorithms, addressing an open research question ~\cite{de2021classification}. 
To do this, we develop two fine-tuning methods and demonstrate their efficacy on both synthetic and image data~\cite{krizhevsky2009learning}.
Our contributions are as follows. 
We (1) develop fine-tuning methods which allow human-AI models to be individual specific and (2) apply this to autonomous driving and image recognition tasks.
% \begin{figure*}
%     \centering
%     \includegraphics[width=400pt]{images/datapoints_5.png}
    
%     \caption{We describe the problem, by noting what type of data is available. Our two fine tuning methods use these data points to learn a rejector and classifier function}
%     \label{fig:datapoints}
% \end{figure*}

==> 2022_neurips_human_machine_decision_collaboration/sections/methods.tex <==
\section{Learning-to-defer algorithms}
We describe three learning-to-defer algorithms, each of which uses data in different ways to develop the function $a$: a non-fine-tuning baseline and two approaches that incorporate fine-tuning. 
\label{sec: methods}
\subsection{Baseline Non-fine-tuning}
We describe the state-of-the-art learning-to-defer algorithm~\cite{mozannar2020consistent}. 
The algorithm first develops a human performance model, $\hat{h}$, which is trained on all human performance data, $w_i$ and $v_i$, and outputs whether a human will answer a data point correctly.
After learning $\hat{h}$, human performance labels are imputed on data points $u_{1} \cdots u_{p}$, so all three data types have human labels. 
Afterward, the learning-to-defer function $a$, and the machine classification function, $m$, are learned simultaneously by reformulating as a $k+1$ classification problem and using a modified cross-entropy loss function that takes into account the cost of deferral. 
See Section ~\cite{mozannar2020consistent} for full details of this approach. 
% \subsection{Semi-supervised learning}
% Our problem can be viewed as an extension of semi-supervised learning, which aims to learn a classifier given both labeled and unlabeled data. 
% In our scenario, we're given both unlabeled image data, image data labeled by other humans, and image data labeled by a specific individual.
% Therefore, the challenge is to incorporate both unlabeled and similarly labeled data effectively. 

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=300pt]{images/accuracy_by_class.png}
%     \caption{Human accuracy varies by the class, ranging from deer at $90\%$ to horses at $98\%$. Machine assistance on deer classes can greatly improve performance. }
%     \label{fig:class}
% \end{figure*}

\subsection{Baseline Fine-tuning} 
We incorporate elements of fine-tuning into the state-of-the-art learning-to-defer algorithm to improve system accuracy for specific individuals.
To do this, we modify the human performance model training, so $\hat{h}$ is first trained for $n$ epochs on aggregate human performance data, $w_i$, then trained for $n \lambda$ epochs on specific human performance data, $v_i$. 
To account for class imbalances, which could skew training due to small fine-tuning dataset size, we introduce a class-weighting scheme, which weights the loss function by the inverse frequency of each class. 
\subsection{Self-training} 
% \begin{figure*}
%     \centering
%     \includegraphics[width=300pt]{images/cifar_pca.png}
%     \caption{We dimensionality reduce CIFAR10 images using the PCA algorithm, and color by human accuracy. Notice that harder images are to the left, and that the difficulty of the image corresponds to the x axis. }
%     \label{fig:pca}
% \end{figure*}


We adopt the self-training algorithm from semi-supervised learning as an alternative to the baseline~\cite{chapelle2009semi}. 
For self-training, we first train a human performance model using specific human data $v_i$.
Using this basic model, we predict labels for the unlabeled data points, $u_{i}$, then select the high confidence predictions.
We use these high confidence points to retrain the model, thereby using unlabeled data points to develop an individual-specific model. 

==> 2022_neurips_human_machine_decision_collaboration/sections/problem.tex <==
\section{Problem Statement}
We define the problem of human-AI collaboration for classification and  learning-to-defer algorithms.
We consider the problem of classifying data points $x_{1}, \ldots, x_{n}$, which have true labels $y_{1}, \ldots, y_{n}$. 
Data points $x_{1}, \ldots, x_{n}$ have human annotations $h_{1}, \ldots, h_{n}$. 
The problem is to develop functions $a$ and $m$ that partition and solve the task, so if $a(x_i) = 0$, the task is solved by a human, and if $a(x_i) = 1$, then the task is solved by a machine, $m$, which is a classification function. 
The objective function is then to maximize 
\begin{equation} 
\sum_{i=0}^{n}  
\begin{cases} 
      h_i=y_i & a(x_i) = 0 \\
      m(x_i)=y_i & a(x_i) = 1
   \end{cases}. 
\end{equation}
To develop the function $a$, we're given the following: 
\begin{enumerate}
    \item Aggregate human data: a set of points (for training) consisting of data points $w_1, \ldots, w_m$, human labels $g_1, \ldots, g_m$ (aggregated across multiple humans), and true labels $z_1, \ldots, z_m$. 
    \item Specific human data: a set of points (for fine-tuning and testing) consisting of data points $v_1, \ldots, v_k$ ($k < m$), human labels from an individual $f_1, \ldots, f_k$, and true labels $t_1, \ldots, t_m$.
    \item Non-human labeled data points: a set of points (for imputing human labels) consisting of data points $u_1, \ldots, u_p$ ($k < m < p$) and truth labels $s_1, \ldots, s_p$.
\end{enumerate}

% Learning-to-defer functions to partition the testing data points, so each is either solved by a human, meaning the predicted label is given by $h(x_i)$, or is solved by a machine (AI), meaning the predicted label is given by $m(x_i)$. 
% The learning-to-defer function, $a$, is either $0$ when data points are solved by humans, or $1$ when solved by machines. 
% Learning-to-defer functions are based on human performance models, $\hat{h}$, which, given a data point, outputs whether a human would answer it correctly. 
% Our aim to maximize overall system accuracy, so if we let $a(x_i)=0$ if a human answers, and $a(x_i)=1$ otherwise, then the objective is to pick a function $a$ that maximizes 



% % Rather than viewing human data as arising from a distribution of skill, we view human data as arising from a distribution of distributions. 
% % That is, each individual has their own distribution of skills, and the parameters for that distribution are itself taken from a distribution. 

% % Following previous work, we aim to learn both the deference function $a$ and the classifier $m$ simultaneously~\cite{mozannar2020consistent}. 
% % These deference functions are based on determining whether humans or AIs are better at a particular data point, $x_i$, which relies on models of human skill. 
% % To learn $a$ and $m$, we consider two types of training points: human-annotated training points and truth-labeled training points.
% % Truth-labeled points are common and serve as training points for a classifier, while human-annotated training points serve to assess human skill at a task. 
% % We have training points, $t_{1} \cdots t_{a}$, with truth labels $s_{1} \cdots s_{a}$, but lack human labels. 
% % We have humans labeled points $c_{1} \cdots c_{l}$ with truth labels $d_{1} \cdots d_{l}$ and human labels $e_{1} \cdots e_{l}$. 
% % We additionally have points from one individual, who annotated points $x_1 \cdots x_n$ with truth labels $y_1 \cdots y_n$ and human labels $z_1 \cdots z_n$. 
% % We consider the first $\frac{n}{2}$ individual-specific points to be for fine-tuning and the last $\frac{n}{2}$ to be for testing. 
% % Therefore, we aim to learn $m$ and $a$ to maximize 


% % % \begin{figure*}
% % %     \centering
% % %   \includegraphics[width=250pt]{images/datapoints_6.png}
% % %   \includegraphics[width=250pt]{images/datapoints_7.png}
% % %     \caption{Our two fine tuning methods. The first uses individual-specific data on top of the human model, while the second uses self training to fine tune the model. }
% % %     \label{fig:fine_tuning}
% % % \end{figure*}

==> 2022_neurips_human_machine_decision_collaboration/sections/related.tex <==
\section{Related Works}
\textbf{Human-AI Collaboration}. Collaboration between humans and machines has been explored in various domains including finance~\cite{nagar2011making} and healthcare~\cite{patel2019human}. 
Collaboration is beneficial as information from both sources can be combined to make decisions~\cite{nagar2011making}. 
However, collaboration has risks, as algorithmic predictions can anchor and bias human predictions~\cite{vaccaro2019effects}. 
This problem is further exacerbated when AI solutions are accompanied by explanations~\cite{bansal2021does}, as humans are more liable to accept explanations regardless of their veracity. 
However, the problem can be mitigated through the development of human mental models, which acknowledge deficits in AI performance~\cite{bansal2019beyond}. 
\\ \\
\textbf{Learning to defer}. One area of research within human-AI collaboration is learning to defer, where AI systems defer to humans when unsure. 
For classification problems, the AI system consists of a rejector, which determines whether or not to defer, and a classifier, which solves the task. 
One strategy is to calculate confidence scores for AI and humans, and defer based on whichever is higher~\cite{raghu2019algorithmic,madras2017predict}. 
However, these confidence-based approaches ignore the interconnectedness of the rejector and classifier by training the classifier independently. Ideally, the classifier should be trained to focus on tasks that are hard for humans, and to solve this, prior work has developed a joint learning algorithm to simultaneously learn a rejector and classifier through the use of a new loss function~\cite{wilder2020learning,mozannar2020consistent}. 
In the case of SVMs, prior work has shown theoretically and experimentally that learning-to-defer algorithms outperform humans and machines separately~\cite{de2021classification}.
Extensions to the learning-to-defer approach include algorithms for multiple experts~\cite{keswani2021towards} and human-initiated deferral~\cite{bansal2021most}. 
Our work most directly builds on prior work by Mozannar et al.~\cite{mozannar2020consistent}, and responds to a call from De et al.~\cite{de2021classification} to develop human-AI collaboration algorithms that can be adapted to specific humans.

==> 2022_neurips_human_machine_decision_collaboration/sections/theory.tex <==
\section{Impact of human models}
We present and prove two theorems detailing the impact of human models.
We first detail our problem setup, then prove our two theorems. 

\subsection{Problem Setup} 
We consider the problem of characterizing $n$ inputs $x_1, x_2 \cdots x_n$, with labels $y_1, y_2, \cdots x_n$.
For each input, humans output a label $h(x_{i})$, with a confidence $c_{H}(x_i)$.
Similarly, for AI-based machines, they output a label $m(x_{i})$ with confidence $c_{M}(x_{i})$. 
We calibrate confidences, so that the calibrated confidence for humans is $g_{H}(c_{H}(x_i))$ and for machines $g_{M}(c_{M}(x_i))$. 
Humans and machines have true confidences, $p_{H}(x_i)$ and $p_M(x_i)$, so that the probability of a human answering $x_i$ correctly is $p_{H}(x_i)$. 
We define calibration so that the distribution of errors after calibration, $p_{H}(x_i)-g_{H}(c_{H}(x_i))$ has $\mu=0$ and $\sigma=\epsilon$ (and similarly for machines). 
In other words, calibrated confidence are centered at the true confidence, with a standard deviation of $\epsilon$. 

We now define the joint human-machine system. 
This system takes in $x_i$, and decides whether to give the problem to humans or machines, based on $g_{H}(c_{H}(x_i))$ and $g_{M}(c_{M}(x_i))$. 

\subsection{Model error rates}
Our first theorem demonstrates the relationship between model calibration and model error. 
\\ 
\textbf{Lemma:} The probability of misclassification is $\leq \frac{2\epsilon^{2}}{(p_{H}(x_i)-p_{M}(x_i))^{2}}$ \\ 
\textbf{Proof:}
Without loss of generality, assume $p_{H}(x_i) > p_{M}(x_i)$. 
The probability of an incorrect classification is $\mathrm{Pr}(g_{H}(c_{H}(x_i))<g_{M}(c_{M}(x_i)))$
Assuming independence between the distributions, we let $X = g_{M}(c_{M}(x_i)) - g_{H}(c_{H}(x_i)) = (g_{M}(c_{M}(x_i)) - p_{M}(x_i)) - (g_{H}(c_{H}(x_i)) - p_{H}(x_i)) + (p_{M}(x_i) - p_{H}(x_i))$, and determine $\mathrm{Pr}(X>0)$. 
$X$ is centered at $p_M(x_i) - p_{H}(x_i)$, so $\mathrm{Pr}(X>0) \leq \mathrm{Pr}(|X-(p_{M}(x_i)-p_{H}-x_{i})| \geq (p_{H}(x_i) -p_{M}(x_i)))$
By Chebyshev's inequality, we find $\mathrm{Pr}(|X-(p_{M}(x_i)-p_{H}(x_i))| \geq (p_{H}(x_i) -p_{M}(x_i))) \leq \frac{2 \epsilon^{2}}{(p_{H}(x_i)-p_{M}(x_i))^{2}}$, as $\mathrm{Var}(X) = 2 \epsilon^{2}$
\\
\\
\begin{comment} 
\subsection{Improvement over independent humans/machines}
\label{sec:lemma2}
We next compare errors due to misclassification with errors arising from only using human or machine predictions. 
\textbf{Lemma:} If neither humans nor AI Pareto dominate, then human-AI combination outperforms either independently \\ 
\textbf{Proof:}
We suppose that, for each $i$, $p_{H}(x_i)$ and $p_{M}(x_i)$ are randomly sampled from the uniform distribution $[a_{h},b_{h}]$ and $[a_{m},b_{m}]$, denoting the range of confidences for humans and machines respectively. 
We suppose that $a_{h} \leq a_{m} \leq b_{h} \leq b_{m}$. 
Note that if the uniform distributions do not intersect, that is, $p_{H}(x_i) > p_{M}(x_i)$ for all $i$, then independent human systems outperform joint systems. 
We wish to find the expected loss due to using only human predictions, which is $\mathrm{Pr}(p_{H}(x_i)<p_{M}(x_i))*E[p_{M}(x_i)-p_{H}(x_i)|p_{H}(x_i)<p_{M}(x_i)]$.
Note that the PDF for each uniform distribution is $\frac{1}{b_{h}-a_{h}}$ and $\frac{1}{b_{m}-a_{m}}$
We find this by evaluating a double integral
\begin{equation}
    \begin{aligned}
        \frac{1}{(b_{h}-a_{h})(b_{m}-a_{m})} \int_{a_{h}}^{b_{m}} \int_{a_{h}}^{x} x-y dy dx \\ 
        =  \frac{(b_{m}-a_{h})(\frac{a_{h}^2}{2} - a{h})+\frac{b_{m}}{6}}{(b_{h}-a_{h})(b_{m}-a_{m})}
    \end{aligned}
\end{equation}

The expected error due to misclassification is $E[\epsilon^{2}/(p_{H}(x_{i}) - p_{M}(x_i)) * (p_{H}(x_{i}) - p_{M}(x_i)] = E[\frac{\epsilon^2}{p_{H}(x_{i})-p_{M}(x_i)}] = \frac{\epsilon^{2}}
{E[p_{H}(x_{i})-p_{M}(x_i)]}$. 
We evaluate the denominator to get 
\begin{equation}
    \begin{aligned}
    \int_{a_{m}}^{b_{m}} \int_{a_{h}}^{x} x-y dy dx + \int_{a_{m}}^{b_{m}} \int_{x}^{b_{h}} y-x dy dx = \\ 
    \frac{6 \epsilon^2 (c-d)}{3d^2-3(b+a)(d) + 3c^2-3(b+a)c+2b^2+2ab+2a^2}
    \end{aligned}
\end{equation}

In essence, this means that if we can reduce $\epsilon$ so that it's sufficiently small, and if humans are not dominant on every questions, then combining humans and machines can outperform either independently. 
\end{comment}

==> lincoln/abstract.tex <==
\begin{abstract}
AI-based systems are used in tandem with humans across a variety of fields including healthcare and criminal justice. 
Maximizing system performance in these situations requires AI to understand the strengths limitations of humans, and allocate tasks accordingly. 
To do this, we build on learning-to-defer models, which allow AI to determine when to defer to humans, to make these models individual specific. 
Doing so allows for finer-grained deference, potentially improving system performance. 
We first outline two strategies for fine tuning, and display the efficacy of individual-specific deference using a synthetic autonomous-vehicle dataset. 
We then conduct experiments using the CIFAR10 image classification task, showing that in some situations, using individual-specific models allows AI to better understand human performance. 
However, we find that this improvement in understanding does not correlate with an improvement in system performance. 
This is potentially due to weak learning algorithms; we propose directions to mitigate this issue and plan for future experiments. 
\end{abstract}

==> lincoln/conclusion.tex <==
\section{Conclusion}
We explore the use of individual-specific human-AI collaboration algorithms. 
We find that the use of individual-specific algorithms can improve expert accuracy rates, and in some cases, improve system performance. 
However, for real experts, improving system performance is difficult due to weaknesses in the learning algorithm. 
We propose future work which rectifies these issues in addition to new experiments. 

==> lincoln/corrupted.tex <==
\section{Corrupted Image recognition}
\subsection{Task Introduction}
What is CIFAR10C? 
\subsection{Data Collection}
How do we collect data for CIFAR10C? 
\subsection{CIFAR10C Data Analysis}
What do machine errors look like on CIFAR10C? What about human errors? We could either have one annotator, or multiple, and fine tune.
\subsection{Experiment Setup}
How do we run the experiment on CIFAR10C. 
\subsection{Results}
What are the results? What does this mean for robustness more generally? 

==> lincoln/discussion.tex <==
\section{Discussion}
\subsection{Limitations}
Our work investigates the use of individual-specific human-AI collaboration algorithms. 
Our results were tested on several annotators and synthetic experts, but could have been expanded, both in terms of the number of trials, and the number of experts. 
Additionally, our semi-supervised learning might not have been robust enough to pick up on expert patterns, and so could be improved through better algorithms. 
In light of this, we discuss future work that builds on our current work. 

\subsection{Future Work}
We explore three avenues for future work. 

\subsubsection{Improved semi-supervised learning algorithms}
As covered in section~\ref{sec: methods}, the problem of incorporating fine tuning to make algorithms individual-specific can be viewed as a form of semi-supervised learning. 
As such, while we have employed self-training algorithms, more sophisticated graph-based algorithms could yield improvements in performance by learning underlying expert patterns. 
Additionally, unlabeled data could be utilized by enforcing an entropy regularization term in the loss function, so to minimize the entropy of unlabeled points while maximizing accuracy on labeled points. 

\subsubsection{Jeopardy Experiments}
To explore the use of human-AI deference algorithms for text datasets, we plan on conducting experiments using the jeopardy question answering dataset~\cite{jeopardy}. 
Individuals vary on skill-set for different types of questions - for example, some people are good at literature, while others are good at science. 
AI models should recognize this, and defer to humans on their strong subjects, while taking over on their weak subjects. 
Doing so potentially requires the use of topic modelling to identify topics, which can be used as inputs to a deep learning model. 
Additionally, surveying expert skill at a topic is a challenge due to incomplete information, as players who might know a topic could fail to buzz in time.
To address this issue, we plan to use some type of imputation to determine confidences on unknown questions. 

\subsubsection{Corrupted Dataset}
Individual-specific fine tuning can be used to explore human robustness on image recognition tasks. 
The CIFAR10C dataset is a corruption of the CIFAR10 dataset, and has been shown to be more difficult for humans~\cite{hendrycks2019robustness}. 
Testing a human-AI collaboration algorithm on this dataset would yield insight into how well human-AI tandems work in the presence of corruptions, and whether humans and AIs are robust to different types of corruptions. 
However, doing so first requires a human-annotated version of the CIFAR10C dataset, which can potentially be collected through MTurk or from volunteers. 
The experiment serves as a way to explore AI predictions when subject to out-of-domain data. 

==> lincoln/driving.tex <==
\section{Motivating Experiments - Autonomous Vehicles}
\label{sec:driving}
Human-AI collaboration naturally arises in the realm of autonomous vehicles, and while the quality of these vehicles has improved recently, they still lag behind humans.
We allow autonomous vehicles to defer to humans depending on environmental circumstances, and show that fine tuning deference algorithms for individual humans reduces trip durations. 
We first develop a synthetic dataset, then describe our results. 

\subsection{Experimental Setup}
We consider the problem of driving a vehicle under rain and darkness conditions. 
Specifically, we consider vehicle deferral for a given driver, $i$, given raining conditions, $0 \leq r \leq 1$, and darkness conditions, $0 \leq d \leq 1$.
Our dataset consists of $n$ total drivers, each of whom have a mean driving time, $\mu \sim \mathrm{Poisson(35)}$, a rain driving time, $\mu_r \sim \mathrm{Poisson(5)}$, and a darkness driving time, $\mu_d \sim \mathrm{Poisson(5)}$. 
Given $\mu$, $\mu_r$, $\mu_d$, the amount of time necessary to drive a trip in conditions $(r,d)$ is distributed according to 

\begin{equation} 
\mathcal{N}(\mu,\sigma) + r \mathcal{N}(\mu_r,\sigma_r) +  d \mathcal{N}(\mu_d,\sigma_d) 
\end{equation} 

We generate $k$ such trips for each driver; for drivers $j \neq i$, the points are for training, while for driver $i$, the points are split equally between fine tuning and testing. 
During deferral, autonomous vehicles have three options: they can defer to humans, drive independent of conditions in time $\mathcal{N}(\mu_a,\sigma_a)$, or dependent on the conditions in time $\mathcal{N}(\mu_b,\sigma_b) + r \mathcal{N} (\mu_x,\sigma_x) + d \mathcal{N} (\mu_y,\sigma_y)$, where $\mu,\sigma$ are constants. 
This forces autonomous vehicles to learn both a rejector and classifier function, emulating the joint classification-deference problem. 
To assist with learning, an additional $l$  unlabeled $(r,d)$ pairs are presented, and time value predictions are imputed, which follows our method from section ~\ref{sec: methods}. 
For our experiments, we use $\sigma=5$, $\sigma_r=\sigma_d=2$, $\mu_a = 45$, $\sigma_a = .001$, $\mu_b = 40$, $\sigma_b = 5$ $\mu_x = \mu_y = 5$, $\sigma_x = \sigma_y = 2$.


\begin{figure*}
    \centering
    \includegraphics[width=400pt]{images/driving.png}
    \caption{Distribution of time taken with/without fine-tuning, and optimally. Each data point represents the average duration when fine tuning on one driver, over $128$ testing trips. Fine tuning out performs not fine tuning by 30 seconds, showing that fine tuning can assist}
    \label{fig:driving}
\end{figure*}

\subsection{Experimental Results}
We generate $k=256$ trips for $n=10$ drivers, and create an additional $l=1024$ unlabeled rides. 
We train an expert prediction network and a rejector function, and compute time taken for each trip. 
We use a simple feed-forward neural network to model both the rejector-classifier, and the human model. 
To analyze the results, we compute two metrics: ideal time, which chooses as if trip durations are known a priori, thereby ignoring randomness, and known mean, which selects deference based on $\mu$ values. 
Both of these serve as lower bounds on average trip duration. 

We simulate $1000$ different sets of $10$ drivers, and for each, compute the average trip duration, plotting them on figure~\ref{fig:driving}. 
We find that, through fine tuning, we can reduce the average trip duration by 30 seconds, while perfectly learning the mean can reduce trip durations by 2 minutes 30 seconds. 
Therefore, fine tuning reduces trip duration error by $20\%$, and our results are significant with $p<.001$. 
While the median between fine tune and no fine tune are close, the averages are wider apart due to large outliers when not fine tuning. 


==> lincoln/image.tex <==
\section{CIFAR Experiments}
We use the CIFAR image recognition task to asses the impact of fine tuning on human-AI collaboration, using both synthetic and real-world human data. 
We discuss our mixed results and propose next steps. 

\subsection{CIFAR10 dataset}
The CIFAR10 image recognition task asks users to classify 32x32 images into one of ten non-overlapping categories~\cite{krizhevsky2009learning}. 
Human performance on the task in the low to mid 90s, while machine performance has exceeded human performance, and is around $99\%$~\cite{foret2020sharpness}. 
To show the efficacy of human-AI collaboration, we reduce the number of training epochs, so machine performance is at $94\%$. 
We begin by analyzing human performance by utilizing the CIFAR10H dataset, where 50 humans label each test image from CIFAR10~\cite{peterson2019human}. 
We find that, while aggregate human performance is in the mid 90s, human performance varies by class label, ranging from deer at $90\%$ to horse at $98\%$ (figure ~\ref{fig:class}). 
Accuracy differences across classes implies that machine takeover on human-weak classes can improve classification, assuming humans and machines have different accuracy profiles, which is also a consequence of section~\ref{sec:lemma1}. 

\subsection{Manifold exploration}
We investigate CIFAR10 images to determine if differences between easy and hard images are learnable. 
To do this, we apply the PCA dimensionality reduction algorithm to images, and analyze the accuracies of dimensionality reduced points.  
We color points by accuracy, binning accuracies into groups rounded to the nearest tenth, and find that accuracy correlates with the PCA x axis. 
The PCA plot hints at the idea that some fundamental component of an image correlates with accuracy, and so identifying easy and hard images is a feasible task. 

\subsection{Synthetic Experts}
To test the effect of fine tuning in a controlled setting, we develop synthetic experts, and consider their effect on human-AI collaboration. 
These experts are parameterized by the value $k$, which indicates perfect accuracy on the first $k$ image classes, and random guesses on the last $10-k$. 
For example, we would expect a $k=10$ expert to achieve $100\%$ accuracy, and a $k=5$ expert to achieve $50\%+50\%\times10\% == 55\%$ accuracy. 
Each synthetic expert annotates $500$ data points, $250$ of which are for fine tuning, and the rest are for testing. 
We use real human data for training, and use synthetic expert for fine tuning. 

We describe our procedure below; the procedure is also described in section~\ref{sec: methods}. 
We begin by training an expert prediction function that predicts expert success on a problem using a WideResNet model, which outputs $0$ if correct, and $1$ otherwise. 
We train on aggregate human data, then fine tune on half the synthetic expert data. 
After training the expert prediction function, we impute predictions on the 50k training labels, and use the combined data to train a rejector. 
The rejector is an 11 class WideResNet model, which outputs 0-9 to predict a class, and 10 to defer. 
We evaluate the rejector by running it over test data points and comparing system accuracy. 
\subsection{Real Annotator Experiments} 
We run experiments to determine the impact of fine tuning on individual annotators. 
Each annotator for the CIFAR10H dataset annotates 200 images; we aim to optimize for these annotators by fine tuning on 100 images and testing on the other 100. 
Our setup is similar to the synthetic experiments, except swapping synthetic with real experts. 
We repeat this for 11 different annotators and asses the impact on system accuracy. 
\subsection{Experimental Setup}
We run both real and synthetic expert experiments, trying $k=0 \cdots 10$ for synthetic experiments, and using 11 different annotators for real annotators. 
We measure deference rate and accuracy on deferences. 
We try three different types of fine tuning: no fine tuning, baseline fine tuning, and self training. 
\subsection{Results}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=200pt]{images/human_model_accuracy_synthetic.png}
    \includegraphics[width=200pt]{images/human_model_accuracy_annotator.png}
    \caption{We plot human model accuracies for synthetic and real annotator collaborations. We find that introducing fine tuning assists human model accuracies for synthetic data but not real annotators. }
    \label{fig:human_accuracy}
\end{figure}
We overview our biggest takeaways from the synthetic and real annotator experiments
\begin{enumerate}
    \item \textbf{Introduction of fine tuning can improve expert prediction} - We see that, in the case of synthetic experts, the introduction of fine tuning improves expert prediction accuracy, particularly for low values of K (figure~\ref{fig:human_accuracy}). 
    However, such a pattern fails to hold when dealing with real annotators, as fine tuning fails to outperform not fine tuning. 
    We believe these results occur due to the situation learnability; synthetic experts pose an easier challenge when compared to real annotators, who have more nuanced strengths and weaknesses. 
    Such results could also be due to dataset sizes, as annotators only have 100 fine tuning points, when compared with 256 for synthetic experts. 
    \item \textbf{Improvements in expert prediction accuracy fail to improve system accuracy} - We see that for both synthetic and real annotator data that improvements in expert prediction accuracy fail to result in system accuracy improvements. 
    This is partially explained by low deference rates leading to reliance on system rather than human classification. 
    However, there still are situations where high deference and expert accuracy rates are not aligned with high system accuracy ,and the reasons why are still unknown. 
    \item \textbf{Deference accuracies are high across the board} - For both no fine tuning and the two types of fine tuning, human accuracy on deferred examples is consistently higher than deferring randomly, showing that expert models successfully learn something about human performance.
    Of note is high deference accuracies for low values of $k$ on synthetic experts with no fine tuning. 
    This result is counter-intuitive, as the lack of fine tuning on experts so different from aggregate humans should imply poor performance. 
    The reason this occurs is unknown and could potentially be due to a bug in the code. 
\begin{figure}[!ht]
    \centering
    \includegraphics[width=200pt]{images/system_accuracy_synthetic.png}
    \includegraphics[width=200pt]{images/system_accuracy_annotator.png}
    \caption{We plot system accuracy for synthetic and real annotator setups. Despite improvements in human accuracy, we find that system accuracy fails to consistently increase when using fine tuning, for both synthetic and real annotators. }
    \label{fig:system_accuracy}
\end{figure}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=200pt]{images/deference_accuracy_synthetic.png}
    \includegraphics[width=200pt]{images/deference_accuracy_annotator.png}
    \caption{We compute accuracy on deferred examples, and find that for synthetic experts, deference accuracy is consistently higher than guessing. However, this is true for both with and without fine tuning, which is strange. }
    \label{fig:human_accuracy}
\end{figure}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=200pt]{images/synthetic_accuracy_improvements.png}
    \caption{We plot how improvements in human accuracy impact system accuracy. We find a generally positive pattern, as improvements in human accuracy lead to improvements in system accuracy, though the effect is not very large, and there is a fair amount of noise. Therefore, improvements in human accuracy might contribute to small improvements in system accuracy, but these trends are incredibly noisy.  }
    \label{fig:human_accuracy}
\end{figure}

\end{enumerate}

\subsection{Discussion} 
Our CIFAR experiment results are largely mixed and demonstrate that the rejector understands human performance, but not sufficiently well to improve system performance. 
We believe the problem is due to the learning algorithm rather than the nature of the problem, as sufficiently good learning algorithms should be able to pickup on differences in accuracy profiles. 
Potential steps to mitigate this issue include the use of graph-based semi supervised learning algorithms, and the expansion of fine tuning datasets. 
We additionally find a tradeoff between the amount of data available, and specificity of data for the model. 
In particular, we have a small amount of individual-specific data, which is a better fit, and a large amount of aggregate human data, which is a worse fit, which leads to fine tuning only assisting in certain scenarios. 


==> lincoln/introduction.tex <==
\section{Introduction}
The rise of neural technologies has led to the adoption of AI-based solutions for human-facing tasks in fields such as health care and criminal justice. 
Examples of this include the COMPAS recidivism algorithm, which uses AI to predict recidivism probabilities for defendants~\cite{washington2018argue}. 
Many times, these algorithms work alongside humans, and are tasked with determining whether to answer a problem or to defer. 
\\
Determining when to defer, also known as learning to defer, is a challenging problem explored by prior work. 
Determining this relies not only on model confidences, but its interpretation of human expertise. 
Numerous studies~\cite{mozannar2020consistent,raghu2019algorithmic,wilder2020learning} have developed methods to learn when to defer based off human and machine uncertainty.
This includes both confidence-based methods~\cite{raghu2019algorithmic} and joint learning methods~\cite{mozannar2020consistent,okati2021differentiable}, which learn rejector and classifier functions simultaneously. 
Other work in this space includes multi-agent deferral~\cite{keswani2021towards} and human initiated deferral~\cite{bansal2021most}. 
\\
While much of the attention has been focused on optimal learning methods, less attention has been focused on understanding human skill. 
Human skill varies between individuals, and so understanding humans skill in aggregate might not be applicable to instances where individual skill differs from aggregate skill. 
Allowing for deference algorithms to be individual-specific can mitigate this problem, allowing for a more nuanced view of human skill, and potentially improving system performance. 
To tackle this problem, we develop two fine tuning methods which allow for human-AI models to be individual-specific.
We prove theoretical bounds on the error when using joint human-AI systems. 
%that, with sufficient knowledge of human and AI skills, human-AI joint models  out-perform humans or AI models independently, motivating the need to understand human skill. 
As a simple example, we develop a synthetic dataset based on autonomous driving, and show that fine tuning for individuals reduces average trip duration. 
We then run experiments comparing performance using different types of fine tuning for the CIFAR10 image recognition task,using both real and synthetic humans~\cite{krizhevsky2009learning}. 
\\
Our contributions are as follows. 
We (1) develop two fine tuning methods which allow for human-AI models to be individual specific, (2) show the application of this model to autonomous driving and image recognition tasks, and (3) prove bounds on the relationship between human-AI calibration error and system error.
\begin{figure*}
    \centering
    \includegraphics[width=400pt]{images/datapoints_5.png}
    
    \caption{We describe the problem, by noting what type of data is available. Our two fine tuning methods use these data points to learn a rejector and classifier function}
    \label{fig:datapoints}
\end{figure*}

==> lincoln/main.tex <==
\input{meta}
\pdfinfo{
/Title (Human-Machine Joint Collaboration)
/Author (Naveen Raman, Michael Yee)
/TemplateVersion (2021.2)
} 


\setcounter{secnumdepth}{2} 
\title{(DRAFT) Human-Machine Joint Collaboration}
\author{
    Naveen Raman \textsuperscript{\rm 1, \rm 2}, Michael Yee \textsuperscript{\rm 1} 
    \\
}
\affiliations{
    \textsuperscript{\rm 1} MIT Lincoln Labs 
    \textsuperscript{\rm 2} University of Maryland, College Park \\
}


\begin{document}

\maketitle

\makeatletter{\renewcommand*{\@makefnmark}{}
\footnotetext{\\ DISTRIBUTION STATEMENT A. Approved for public release. Distribution is unlimited. \\ \\ This material is based upon work supported by the Under Secretary of Defense for Research and Engineering under Air Force Contract No. FA8702-15-D-0001. Any opinions, findings, conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the Under Secretary of Defense for Research and Engineering.}\makeatother}

\input{sections/abstract}
\input{sections/introduction}
\input{sections/related}
\input{sections/problem}
\input{sections/methods}
\input{sections/theory}
\input{sections/driving}
\input{sections/image}
\input{sections/discussion}
\input{sections/conclusion}

\clearpage
\bibliographystyle{aaai}
\bibliography{references.bib}

\end{document}



==> lincoln/methods.tex <==
\section{Learning algorithms}
We describe a learning algorithm to learn rejectors and classifiers jointly, then describe our two fine tuning methods. 
\label{sec: methods}
\subsection{State of the art human-AI collaboration}
We describe the state of the art human-AI collaboration algorithm, taken from prior work~\cite{mozannar2020consistent}. 
The algorithm does not fine tune on human specific data, and so $n=0$. 
Instead it trains and tests on different splits of the aggregate human data. 
The algorithm proceeds as follows: we first train an artificial  human, $\hat{h}$ from human performance on some subset of the human labeled data, $c_1 \cdots c_b$ with human predictions $e_1 \cdots e_b$, using $c_{b+1} \cdots c_{l}$ for testing. 
Given an input, $c_i$, the function $\hat{h{(c_i)}}$ learns whether a human will answer $c_i$ correctly, returning 0 if the do, and 1 if they don't. 
After learning on $c_1 \cdots c_b$, imputed labels are generated for the whole training set by running $\hat{h}$ over $t_{1} \cdots t_n$. 
Imputation allows for predicted human labels on all test points, which is used when training $m$, the classifier, and $a$, the rejector. 
To improve system performance, $a$ and $m$ are learned simultaneously, so if the classification problem is for $k$-classes, then we learn a $k+1$ classification function, where the ${k+1}^{\textrm{st}}$ class indicates deference to humans. 
For each data point, predictions are made using the augmented machine function (k+1 classes) $\bar{m}$, and then optimized over a modified cross-entropy loss function~\cite{mozannar2020consistent}.
The loss function asses a penalty of $\alpha$ for deferring to humans, and a penalty of $1$ for incorrect predictions. 
After training using this loss function, the augmented machine function, $\bar{m}$, is run over the test dataset, $c_{b+1} \cdots c_{l}$, and evaluated based on system accuracy and loss. 
Full details of this algorithm is found in past work~\cite{mozannar2020consistent}. 
\subsection{Semi-supervised learning}
Our problem can be viewed as an extension of semi supervised learning, which aims to learn a classifier given both labeled and unlabeled data. 
In our scenario, we're given both unlabeled image data, image data labeled by other humans, and image data labeled by a specific individual.
Therefore, the challenge is to incorporate both unlabeled and similarly labeled data in an effective manner. 

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=300pt]{images/accuracy_by_class.png}
    \caption{Human accuracy varies by the class, ranging from deer at $90\%$ to horses at $98\%$. Machine assistance on deer classes can greatly improve performance. }
    \label{fig:class}
\end{figure*}

\subsection{Baseline Fine tuning} 
We incorporate elements of fine tuning into the baseline methodology to improve system accuracy for specific humans. 
We primarily modify the training loop by adding an extra an extra loop to train on the fine tuning set, $x_1 \cdots x_{n/2}$. 
To account for class imbalances, which could skew training due to small fine tuning dataset size, we introduce a class-weighting scheme, which weights the loss function by the inverse frequency of each class. 
\subsection{Self Training} 
\begin{figure*}
    \centering
    \includegraphics[width=300pt]{images/cifar_pca.png}
    \caption{We dimensionality reduce CIFAR10 images using the PCA algorithm, and color by human accuracy. Notice that harder images are to the left, and that the difficulty of the image corresponds to the x axis. }
    \label{fig:pca}
\end{figure*}


We adopt the self training algorithm from semi supervised learning as an alternative to the baseline~\cite{chapelle2009semi}. 
For self training, we first train a classifier using $x_1 \cdots x_{n/2}$. 
Using this basic classifier, we predict labels for the unlabeled data points, $t_{1} \cdots t_{a}$, then select the high confidence predictions. 
We use these high confidence points to retrain the classifier, generating a better classifier in the process. 
The advantage of self training is that it uses unlabeled data points to develop a better classifier, leveraging all the available data. 
We employ both baseline fine tuning and self training as fine tuning mechanisms for our image experiments. 
We present a pictorial representation of both algorithms in figure~\ref{fig:fine_tuning}. 

==> lincoln/problem.tex <==
\section{Problem Statement}
We define the problem of human-AI collaboration for classification. 
That is, given a classification task, $T$, which consists of data points $x_{1} \cdots x_{n}$, and human and AI agents, we consider the problem of apportioning $x_{1} \cdots x_{n}$ to maximize system performance. 
Each point is solved by a human, $h(x_i)$, or a machine, $m(x_i)$. 
Our aim to maximize overall system accuracy, so if we let $a(x_i)=0$ if a human answers, and $a(x_i)=1$ otherwise.  

Rather than viewing human data as arising from a distribution of skill, we view human data as arising from a distribution of distributions. 
That is, each individual has their own distribution of skills, and the parameters for that distribution are itself taken from a distribution. 
We make these distributions explicit in section~\ref{sec:driving}, and provide a visual of these data points in figure~\ref{fig:datapoints}. 

Following previous work, we aim to learn both the deference function $a$ and the classifier $m$ simultaneously~\cite{mozannar2020consistent}. 
To learn $a$ and $m$, we consider two types of training points: human-annotated training points and truth-labeled training points.
Truth-labeled points are common, and serve as training points for a classifier, while human-annotated training points serve to assess human skill at a task. 
We have training points, $t_{1} \cdots t_{a}$, with truth labels $s_{1} \cdots s_{a}$, but lack human labels. 
We have humans labeled points $c_{1} \cdots c_{l}$ with truth labels $d_{1} \cdots d_{l}$ and human labels $e_{1} \cdots e_{l}$. 
We additionally have points from one individual, who annotated points $x_1 \cdots x_n$ with truth labels $y_1 \cdots y_n$ and human labels $z_1 \cdots z_n$. 
We consider the first $\frac{n}{2}$ individual-specific points to be for fine tuning, and the last $\frac{n}{2}$ to be for testing. 
Therefore, we aim to learn $m$ and $a$ to maximize 
\begin{equation} 
\sum_{i=\frac{n}{2}}^{n}  
\begin{cases} 
      h(x_i)=y_i & a(x_i) = 0 \\
      m(x_i)=y_i & a(x_i) = 1  
   \end{cases}
\end{equation}
We describe the state of the art solution, which lacks fine tuning, then describe our two solutions which use fine tuning. 
\begin{figure*}
    \centering
   \includegraphics[width=250pt]{images/datapoints_6.png}
  \includegraphics[width=250pt]{images/datapoints_7.png}
    \caption{Our two fine tuning methods. The first uses individual-specific data on top of the human model, while the second uses self training to fine tune the model. }
    \label{fig:fine_tuning}
\end{figure*}


==> lincoln/related.tex <==
\section{Related Works}
\textbf{Human-AI Collaboration} - Collaboration between humans and machines has been explored in various domains including finance~\cite{nagar2011making} and healthcare~\cite{patel2019human}. 
Collaboration is beneficial as information from both sources can be combined to make decisions~\cite{nagar2011making}. 
However, collaboration has risks, as algorithmic predictions can anchor and bias human predictions~\cite{vaccaro2019effects}. 
This problem is further exacerbated when AI solutions are accompanied with explanations~\cite{bansal2021does}, as humans are more liable to accept explanations regardless of its veracity. 
However, the problem can be mitigated through the development of human mental models, which acknowledge deficits in AI performance~\cite{bansal2019beyond}. 
The lack of algorithmic transparency makes it difficult for humans to ascertain liability to AI models, complicating the legality of algorithmic decision making~\cite{williams2019rethinking}. \\ \\
\textbf{Learning to defer} - One area of research within human-AI collaboration is learning to defer algorithms, where AI systems defer to humans when unsure. 
For classification problem, the AI system consists of a rejector, which determines deference, and classification, which solves the task. 
One deference strategy is to calculate confidence scores for AI and humans, and defer based on whichever is higher~\cite{raghu2019algorithmic,madras2017predict}. 
However, these approaches ignore the interconnectedness of the rejector and classifier, as AI systems should focus on tasks that are hard for humans, and to solve this, prior work has developed a joint learning algorithm to simultaneously learn a rejector and classifier through the use of a new loss function~\cite{wilder2020learning,mozannar2020consistent}. 
Prior work has shown that learning to defer algorithms are proven to outperform humans and machines separately in the case of SVMs~\cite{de2021classification}. 
Extensions to the learning to defer algorithm include algorithms for multiple experts~\cite{keswani2021towards} and for human-initiated deferral~\cite{bansal2021most}. 
Our work most directly builds on work by~\citet{mozannar2020consistent}, and answers an open problem from~\citet{de2021classification} to develop human-AI collaboration algorithms for specific humans via fine-tuning


==> lincoln/text.tex <==
\section{Jeopardy Question Answering}
We extend our human-machine collaboration to a text-based question-answering task. 

\subsection{Dataset}
We use the Jeopardy! dataset to determine human and machine performance on question answering. 
We train a BERT-based model to predict human accuracy (and response time?) based on responses to jeopardy questions. 

\subsection{Data analysis}
We look at the data we collected, and the errors made by humans. 

\subsection{Experiment Setup}
We compare joint human-machine models to human and machine-only model on the text dataset, and also see how well we can fine tune. 

\subsection{Experiment Results} 
We find that, for both image and text-based systems, the inclusion of a human in the loop improves system accuracy. 

==> lincoln/theory.tex <==
\section{Impact of human models}
We present and prove two theorems detailing the impact of human models.
We first detail our problem setup, then prove our two theorems. 

\subsection{Problem Setup} 
We consider the problem of characterizing $n$ inputs $x_1, x_2 \cdots x_n$, with labels $y_1, y_2, \cdots x_n$.
For each input, humans output a label $h(x_{i})$, with a confidence $c_{H}(x_i)$.
Similarly, for AI-based machines, they output a label $m(x_{i})$ with confidence $c_{M}(x_{i})$. 
We calibrate confidences, so that the calibrated confidence for humans is $g_{H}(c_{H}(x_i))$ and for machines $g_{M}(c_{M}(x_i))$. 
Humans and machines have true confidences, $p_{H}(x_i)$ and $p_M(x_i)$, so that the probability of a human answering $x_i$ correctly is $p_{H}(x_i)$. 
We define calibration so that the distribution of errors after calibration, $p_{H}(x_i)-g_{H}(c_{H}(x_i))$ has $\mu=0$ and $\sigma=\epsilon$ (and similarly for machines). 
In other words, calibrated confidence are centered at the true confidence, with a standard deviation of $\epsilon$. 

We now define the joint human-machine system. 
This system takes in $x_i$, and decides whether to give the problem to humans or machines, based on $g_{H}(c_{H}(x_i))$ and $g_{M}(c_{M}(x_i))$. 

\subsection{Model error rates}
Our first theorem demonstrates the relationship between model calibration and model error. 
\\ 
\textbf{Lemma:} The probability of misclassification is $\leq \frac{2\epsilon^{2}}{(p_{H}(x_i)-p_{M}(x_i))^{2}}$ \\ 
\textbf{Proof:}
Without loss of generality, assume $p_{H}(x_i) > p_{M}(x_i)$. 
The probability of an incorrect classification is $\mathrm{Pr}(g_{H}(c_{H}(x_i))<g_{M}(c_{M}(x_i)))$
Assuming independence between the distributions, we let $X = g_{M}(c_{M}(x_i)) - g_{H}(c_{H}(x_i)) = (g_{M}(c_{M}(x_i)) - p_{M}(x_i)) - (g_{H}(c_{H}(x_i)) - p_{H}(x_i)) + (p_{M}(x_i) - p_{H}(x_i))$, and determine $\mathrm{Pr}(X>0)$. 
$X$ is centered at $p_M(x_i) - p_{H}(x_i)$, so $\mathrm{Pr}(X>0) \leq \mathrm{Pr}(|X-(p_{M}(x_i)-p_{H}-x_{i})| \geq (p_{H}(x_i) -p_{M}(x_i)))$
By Chebyshev's inequality, we find $\mathrm{Pr}(|X-(p_{M}(x_i)-p_{H}(x_i))| \geq (p_{H}(x_i) -p_{M}(x_i))) \leq \frac{2 \epsilon^{2}}{(p_{H}(x_i)-p_{M}(x_i))^{2}}$, as $\mathrm{Var}(X) = 2 \epsilon^{2}$
\\
\\
\begin{comment} 
\subsection{Improvement over independent humans/machines}
\label{sec:lemma2}
We next compare errors due to misclassification with errors arising from only using human or machine predictions. 
\textbf{Lemma:} If neither humans nor AI Pareto dominate, then human-AI combination outperforms either independently \\ 
\textbf{Proof:}
We suppose that, for each $i$, $p_{H}(x_i)$ and $p_{M}(x_i)$ are randomly sampled from the uniform distribution $[a_{h},b_{h}]$ and $[a_{m},b_{m}]$, denoting the range of confidences for humans and machines respectively. 
We suppose that $a_{h} \leq a_{m} \leq b_{h} \leq b_{m}$. 
Note that if the uniform distributions do not intersect, that is, $p_{H}(x_i) > p_{M}(x_i)$ for all $i$, then independent human systems outperform joint systems. 
We wish to find the expected loss due to using only human predictions, which is $\mathrm{Pr}(p_{H}(x_i)<p_{M}(x_i))*E[p_{M}(x_i)-p_{H}(x_i)|p_{H}(x_i)<p_{M}(x_i)]$.
Note that the PDF for each uniform distribution is $\frac{1}{b_{h}-a_{h}}$ and $\frac{1}{b_{m}-a_{m}}$
We find this by evaluating a double integral
\begin{equation}
    \begin{aligned}
        \frac{1}{(b_{h}-a_{h})(b_{m}-a_{m})} \int_{a_{h}}^{b_{m}} \int_{a_{h}}^{x} x-y dy dx \\ 
        =  \frac{(b_{m}-a_{h})(\frac{a_{h}^2}{2} - a{h})+\frac{b_{m}}{6}}{(b_{h}-a_{h})(b_{m}-a_{m})}
    \end{aligned}
\end{equation}

The expected error due to misclassification is $E[\epsilon^{2}/(p_{H}(x_{i}) - p_{M}(x_i)) * (p_{H}(x_{i}) - p_{M}(x_i)] = E[\frac{\epsilon^2}{p_{H}(x_{i})-p_{M}(x_i)}] = \frac{\epsilon^{2}}
{E[p_{H}(x_{i})-p_{M}(x_i)]}$. 
We evaluate the denominator to get 
\begin{equation}
    \begin{aligned}
    \int_{a_{m}}^{b_{m}} \int_{a_{h}}^{x} x-y dy dx + \int_{a_{m}}^{b_{m}} \int_{x}^{b_{h}} y-x dy dx = \\ 
    \frac{6 \epsilon^2 (c-d)}{3d^2-3(b+a)(d) + 3c^2-3(b+a)c+2b^2+2ab+2a^2}
    \end{aligned}
\end{equation}

In essence, this means that if we can reduce $\epsilon$ so that it's sufficiently small, and if humans are not dominant on every questions, then combining humans and machines can outperform either independently. 
\end{comment}

==> meta.tex <==
\usepackage{neurips_2021}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors


==> sections/discussion.tex <==
\section{Discussion}
\subsection{Limitations}
Our work investigates the use of individual-specific human-AI collaboration algorithms. 
Our results were tested on several annotators and synthetic experts, but could have been expanded, both in terms of the number of trials, and the number of experts. 
Additionally, our semi-supervised learning might not have been robust enough to pick up on expert patterns, and so could be improved through better algorithms. 
In light of this, we discuss future work that builds on our current work. 

\subsection{Future Work}
We explore three avenues for future work. 

\subsubsection{Improved semi-supervised learning algorithms}
As covered in section~\ref{sec: methods}, the problem of incorporating fine tuning to make algorithms individual-specific can be viewed as a form of semi-supervised learning. 
As such, while we have employed self-training algorithms, more sophisticated graph-based algorithms could yield improvements in performance by learning underlying expert patterns. 
Additionally, unlabeled data could be utilized by enforcing an entropy regularization term in the loss function, so to minimize the entropy of unlabeled points while maximizing accuracy on labeled points. 

\subsubsection{Jeopardy Experiments}
To explore the use of human-AI deference algorithms for text datasets, we plan on conducting experiments using the jeopardy question answering dataset~[\cite{jeopardy}]. 
Individuals vary on skill-set for different types of questions - for example, some people are good at literature, while others are good at science. 
AI models should recognize this, and defer to humans on their strong subjects, while taking over on their weak subjects. 
Doing so potentially requires the use of topic modelling to identify topics, which can be used as inputs to a deep learning model. 
Additionally, surveying expert skill at a topic is a challenge due to incomplete information, as players who might know a topic could fail to buzz in time.
To address this issue, we plan to use some type of imputation to determine confidences on unknown questions. 

\subsubsection{Corrupted Dataset}
Individual-specific fine tuning can be used to explore human robustness on image recognition tasks. 
The CIFAR10C dataset is a corruption of the CIFAR10 dataset, and has been shown to be more difficult for humans~[\cite{hendrycks2019robustness}]. 
Testing a human-AI collaboration algorithm on this dataset would yield insight into how well human-AI tandems work in the presence of corruptions, and whether humans and AIs are robust to different types of corruptions. 
However, doing so first requires a human-annotated version of the CIFAR10C dataset, which can potentially be collected through MTurk or from volunteers. 
The experiment serves as a way to explore AI predictions when subject to out-of-domain data. 

==> sections/theory.tex <==
\section{Impact of human models}
We present and prove two theorems detailing the impact of human models.
We first detail our problem setup, then prove our two theorems. 

\subsection{Problem Setup} 
We consider the problem of characterizing $n$ inputs $x_1, x_2 \cdots x_n$, with labels $y_1, y_2, \cdots x_n$.
For each input, humans output a label $h(x_{i})$, with a confidence $c_{H}(x_i)$.
Similarly, for AI-based machines, they output a label $m(x_{i})$ with confidence $c_{M}(x_{i})$. 
We calibrate confidences, so that the calibrated confidence for humans is $g_{H}(c_{H}(x_i))$ and for machines $g_{M}(c_{M}(x_i))$. 
Humans and machines have true confidences, $p_{H}(x_i)$ and $p_M(x_i)$, so that the probability of a human answering $x_i$ correctly is $p_{H}(x_i)$. 
We define calibration so that the distribution of errors after calibration, $p_{H}(x_i)-g_{H}(c_{H}(x_i))$ has $\mu=0$ and $\sigma=\epsilon$ (and similarly for machines). 
In other words, calibrated confidence are centered at the true confidence, with a standard deviation of $\epsilon$. 

We now define the joint human-machine system. 
This system takes in $x_i$, and decides whether to give the problem to humans or machines, based on $g_{H}(c_{H}(x_i))$ and $g_{M}(c_{M}(x_i))$. 

\subsection{Model error rates}
Our first theorem demonstrates the relationship between model calibration and model error. 
\\ 
\textbf{Lemma:} The probability of misclassification is $\leq \frac{2\epsilon^{2}}{(p_{H}(x_i)-p_{M}(x_i))^{2}}$ \\ 
\textbf{Proof:}
Without loss of generality, assume $p_{H}(x_i) > p_{M}(x_i)$. 
The probability of an incorrect classification is $\mathrm{Pr}(g_{H}(c_{H}(x_i))<g_{M}(c_{M}(x_i)))$
Assuming independence between the distributions, we let $X = g_{M}(c_{M}(x_i)) - g_{H}(c_{H}(x_i)) = (g_{M}(c_{M}(x_i)) - p_{M}(x_i)) - (g_{H}(c_{H}(x_i)) - p_{H}(x_i)) + (p_{M}(x_i) - p_{H}(x_i))$, and determine $\mathrm{Pr}(X>0)$. 
$X$ is centered at $p_M(x_i) - p_{H}(x_i)$, so $\mathrm{Pr}(X>0) \leq \mathrm{Pr}(|X-(p_{M}(x_i)-p_{H}-x_{i})| \geq (p_{H}(x_i) -p_{M}(x_i)))$
By Chebyshev's inequality, we find $\mathrm{Pr}(|X-(p_{M}(x_i)-p_{H}(x_i))| \geq (p_{H}(x_i) -p_{M}(x_i))) \leq \frac{2 \epsilon^{2}}{(p_{H}(x_i)-p_{M}(x_i))^{2}}$, as $\mathrm{Var}(X) = 2 \epsilon^{2}$
\\
\\
\begin{comment} 
\subsection{Improvement over independent humans/machines}
\label{sec:lemma2}
We next compare errors due to misclassification with errors arising from only using human or machine predictions. 
\textbf{Lemma:} If neither humans nor AI Pareto dominate, then human-AI combination outperforms either independently \\ 
\textbf{Proof:}
We suppose that, for each $i$, $p_{H}(x_i)$ and $p_{M}(x_i)$ are randomly sampled from the uniform distribution $[a_{h},b_{h}]$ and $[a_{m},b_{m}]$, denoting the range of confidences for humans and machines respectively. 
We suppose that $a_{h} \leq a_{m} \leq b_{h} \leq b_{m}$. 
Note that if the uniform distributions do not intersect, that is, $p_{H}(x_i) > p_{M}(x_i)$ for all $i$, then independent human systems outperform joint systems. 
We wish to find the expected loss due to using only human predictions, which is $\mathrm{Pr}(p_{H}(x_i)<p_{M}(x_i))*E[p_{M}(x_i)-p_{H}(x_i)|p_{H}(x_i)<p_{M}(x_i)]$.
Note that the PDF for each uniform distribution is $\frac{1}{b_{h}-a_{h}}$ and $\frac{1}{b_{m}-a_{m}}$
We find this by evaluating a double integral
\begin{equation}
    \begin{aligned}
        \frac{1}{(b_{h}-a_{h})(b_{m}-a_{m})} \int_{a_{h}}^{b_{m}} \int_{a_{h}}^{x} x-y dy dx \\ 
        =  \frac{(b_{m}-a_{h})(\frac{a_{h}^2}{2} - a{h})+\frac{b_{m}}{6}}{(b_{h}-a_{h})(b_{m}-a_{m})}
    \end{aligned}
\end{equation}

The expected error due to misclassification is $E[\epsilon^{2}/(p_{H}(x_{i}) - p_{M}(x_i)) * (p_{H}(x_{i}) - p_{M}(x_i)] = E[\frac{\epsilon^2}{p_{H}(x_{i})-p_{M}(x_i)}] = \frac{\epsilon^{2}}
{E[p_{H}(x_{i})-p_{M}(x_i)]}$. 
We evaluate the denominator to get 
\begin{equation}
    \begin{aligned}
    \int_{a_{m}}^{b_{m}} \int_{a_{h}}^{x} x-y dy dx + \int_{a_{m}}^{b_{m}} \int_{x}^{b_{h}} y-x dy dx = \\ 
    \frac{6 \epsilon^2 (c-d)}{3d^2-3(b+a)(d) + 3c^2-3(b+a)c+2b^2+2ab+2a^2}
    \end{aligned}
\end{equation}

In essence, this means that if we can reduce $\epsilon$ so that it's sufficiently small, and if humans are not dominant on every questions, then combining humans and machines can outperform either independently. 
\end{comment}
